Heroes: Lightweight Federated Learning with Neural Composition and Adaptive Local Update in Heterogeneous Edge Networks

Federated Learning (FL) enables distributed clients to collaboratively train models without exposing their private data. However, it is difficult to implement efficient FL due to limited resources. Most existing works compress the transmitted gradients or prune the global model to reduce the resource cost, but leave the compressed or pruned parameters under-optimized, which degrades the training performance. To address this issue, the neural composition technique constructs size-adjustable models by composing low-rank tensors, allowing every parameter in the global model to learn the knowledge from all clients. Nevertheless, some tensors can only be optimized by a small fraction of clients, thus the global model may get insufficient training, leading to a long completion time, especially in heterogeneous edge scenarios. To this end, we enhance the neural composition technique, enabling all parameters to be fully trained. Further, we propose a lightweight FL framework, called Heroes, with enhanced neural composition and adaptive local update. A greedy-based algorithm is designed to adaptively assign the proper tensors and local update frequencies for participating clients according to their heterogeneous capabilities and resource budgets. Extensive experiments demonstrate that Heroes can reduce traffic consumption by about 72.05\% and provide up to 2.97$\times$ speedup compared to the baselines.

==> content/trash.tex <==
% In this section, we define the problem of heterogeneity-aware FL with adaptive neural compostion and gredient compression. Let $t_{i}^{k, cp}$ denote the computation time for local updating of client $i$ at round $k$, which is related to the size of coefficient obviously. The larger the coefficient is, the more parameters the composed model will have, leading to longer local computation time. Considering the upload speed is usually much smaller than the download speed in FL and the parameters download time is negligible, we focus on the gredients upload time. Suppose that the gredients size of shared basis and full coefficient are $B_{v}$ and $B_{u}$, respectively, the communication time of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cm} = \frac{r_{i}^{k} (B_{v} + p_{i}^{k} B_{u}) } {b_{i}^{k}}
% \end{equation}
% where $c_{i}^{k}$ represents the upload bandwidth of client $i$ at round $k$, which is heterogeneous among clients and can change dynamically in different rounds. We define the completion time of client $i$ at round $k$ as follows:
% \begin{equation}
%     t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}
% \end{equation}
% Due to the synchronization barrier of FL, the round time (\ie, duration between two successive
% training rounds) depends on the slowest client, which can be expressed as:
% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{N}} \ t_{i}^{k}
% \end{equation}

% Our goal is to determine the optimal coefficient pruning ratios and gredients compression ratios for each client every round, so as to accelerate the training process in the heterogeneous FL setting. Accordingly, we formulate the joint optimization problem as follows:

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \epsilon \\
%     p_{i}^{k} \in \mathcal{P}, &\forall i, \forall k \\
%     0 < r_{i}^{k} \leq  1, & \forall i, \forall k 
%     \end{cases}
% \end{equation}

% The first inequality expresses the convergence requirement, where $\epsilon$ (a positive constant close to zero) is the convergence threshold of the training loss after $K$ rounds. The second set of inequalities bounds the feasible range of coefficient pruning ratios, while the third set of inequalities bounds that of gredient compression ratios.

% In this section, we define the problem of heterogeneity-aware FL with adaptive client selection and neural composition. Let $g(x_{i}^{k, h}, p_{i}^{k})$ represent the number of CPU cycles required to perform one local update, which is related to the size of coefficient. The larger the coefficient is (\ie, the more parameters the composed model have), the more CPU cycles it required to process a batch of data samples. Thus, the computation the of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cp} = \frac{\sum_{h=1}^{H} g(x_{i}^{k, h}, p_{i}^{k})} {c_{i}^{k}}
% \end{equation}

% where $c_{i}^{k}$ denote the CPU-cycle frequency for local training in round $k$. For the communication time, considering the upload speed is usually much smaller than the download speed in FL and the parameters download time can be negligible, we focus on the upload time. Suppose that the size of shared basis and full coefficient are $B_{v}$ and $B_{u}$, respectively, the communication time of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cm} = \frac{(B_{v} + p_{i}^{k}B_{u}) } {b_{i}^{k}}
% \end{equation}

% where $c_{i}^{k}$ represents the upload bandwidth of client $i$ at round $k$, which is heterogeneous among clients and can change dynamically in different rounds. Due to the synchronization barrier of FL, the round time (\ie, duration between two successive training rounds) depends on the slowest client, which can be expressed as:

% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{M}^{k}} \ t_{i}^{k}
% \end{equation}


% where $t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}$. Our goal is to select the clients involved in FL based on the statistical heterogeneity and determine the optimal size of coefficient for those selected clients, so as to accelerate the training process in the heterogeneous FL setting. Accordingly, we formulate the joint optimization problem as follows:

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \epsilon \\
%     p_{i}^{k} \in \mathcal{P}, &\forall i, \forall k \\
%     |\mathcal{M}^{k}| = M, & \forall k 
%     \end{cases}
% \end{equation}

% The first inequality expresses the convergence requirement, where $\epsilon$ (a positive constant close to zero) is the convergence threshold of the training loss after $K$ rounds. The second set of inequalities bounds the feasible range of coefficient pruning ratios. The third set of inequalities indicates that the PS selects $M$ clients participating in training at each round.

% $c_{i}^{p}$ is the computing resource consumption of one local iteration.
% $b_{v}$ and $b_{u}$

% \begin{equation}
%     t_{i}^{k, cp} = \frac{\sum_{h=1}^{\tau_{i}^{k}} g(x_{i}^{k, h}, p_{i}^{k})} {c_{i}^{k}}
% \end{equation}

% \begin{equation}
%     t_{i}^{k, cm} = \frac{(B_{v} + p_{i}^{k}B_{u}) } {b_{i}^{k}}
% \end{equation}

% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{N}} \ t_{i}^{k}
% \end{equation}

% \begin{equation}
%     t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}
% \end{equation}

% \begin{equation}
%     \mathcal{W}^{k} = \frac{1}{N} \sum_{i = 1}^{N} (t^{k} - t^{k}_{i})
% \end{equation}

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \xi  \\
%     \sum_{k = 1}^{K} \sum_{i = 1}^{N} (b_{i, v} + b_{i, u} \cdot p_{i}^{k}) \leq B  \\
%     \sum_{k = 1}^{K} \sum_{i = 1}^{N} \tau_{i}^{k} \cdot p_{i}^{k}c_{i} \leq C 
%     \end{cases}
% \end{equation}


% t_{i}^{k} = \frac{\tau_{i}^{k} g(V^{k} \cdot U^{k}_{p_{i}})} {c_{i}^{k}} + \frac{h(V) + h(U^{k}_{p_{i}}) } {b_{i}^{k}}, & \forall i, k \\

% \subsection{Federated Learning Basics}
% Consider a loose federation of $N$ clients $\mathcal{N} = \{1, 2, \cdots, N \}$ coordinated by the PS.
% Each client $n \in \mathcal{N}$ holds its local dataset $D_{n} = \{\zeta_{i}^{n}\}_{i=1}^{|D_{n}|}$, where $\zeta_{i}$ denotes a data sample from $D_{n}$.
% Further, we represent the loss function as $\mathcal{L}(\mathbf{x}; \zeta)$, which measures how well the model $\mathbf{x}$ perform on data sample $\zeta$.
% Therefore, the local loss function of client $n$ is defined as:

% \begin{equation}
%     F_{n}(\mathbf{x}) \triangleq \mathbb{E}_{\zeta \thicksim D_{n}} [\mathcal{L}(\mathbf{x}; \zeta)] 
% \end{equation}

% The global loss function is a linear combination of all $N$ clients, and the goal of FL is to train a high-quality model $\mathbf{x}^{*}$ to minimize the value of global loss function, which can be defined as follows:

% \begin{equation} \label{eq:fl_goal}
%     \mathbf{x}^{*} \triangleq  \mathop{\arg\min}_{\mathbf{x}} F(\mathbf{x}) = \mathop{\arg\min}_{\mathbf{x}} \frac{1}{N} \sum_{n=1}^{N} F_{n} (\mathbf{x})
% \end{equation}

% FedAvg \cite{mcmahan2017communication} is the pioneer and also the most widely used FL method to solve the problem in Eq. \eqref{eq:fl_goal}.
% In each round $h \in \{1, 2, \cdots, H\}$, the PS randomly selects $K$ clients to participate in training and sends the global model $\mathbf{x}^{h}$ to the selected clients $\mathcal{N}^{h} \subseteq  \mathcal{N}$.
% Then, each client $n \in \mathcal{N}^{h}$ performs local update for $\tau$ iterations.
% Let $\mathbf{x}^{h}_{n} (t)$ denote the local model of client $n$ at iteration $t$ in round $h$.
% For the mini-batch stochastic gradient descent (SGD) algorithm, a local update step can be expressed as follows:

% \begin{equation}
%     \mathbf{x}^{h}_{n} (t+1) = \mathbf{x}^{h}_{n} (t) - \eta \nabla F_{n} (\mathbf{x}^{h}_{n} (t); \xi_{n}^{h, t})
% \end{equation}
% where $\xi_{n}^{h, t}$ denotes a random data batch from the local dataset $D_{n}$ and $\eta$ is the learning rate.
% Finally, the PS collects the updated model $\mathbf{x}^{h}_{n}$ from the participating clients and aggregate them to the latest global model for further training, \ie, $ \mathbf{x}^{h+1} = \frac{1}{N} \sum_{n=1}^{N} \mathbf{x}^{h}_{n} (\tau) $.




% \subsection{Impact of model width}

% As the most common terminal device, mobile phones are the primary data source and usually participate in training as clients.
% However, in practice, these phones are generally resource-constrained with poor computing power, so that they may not be able to afford the overhead to train the complete model.
% Therefore, it is necessary to reduce the model complexity for these poor clients, which can be achieved by reducing the model's depth (\ie, number of layers) or width (\ie, number of hidden channels) \cite{diao2020heterofl, horvath2021fjord, kim2023depthfl}.
% In this work, we adjust the model complexity by modulating the model width, which can reduce parameters and memory footprint during training more effectively compared to reduing model depth \cite{mei2022resource}.

% We can significantly reducing the computing complexities and training overhead of a DNN model, but it usually comes with performance degradation.
% To verify this phenomenon, we construct a CNN model with three 3$\times$3 convolutional layers and one fully-connected layer.
% We reduce the number of hidden channels in each layer by 0.25, 0.5, 0.75 and 1.0 times, respectively, and train these models in different width over CIFAR-10 to record their training overhead and test accuracy.
% The results shown in Table. xx indicate that the smaller the model width, the less training overhead, but the lower the accuracy.
% For instance, xxxx.
% To minimize the performance degradation, the model width should be as large as possible within the clients' computing power.

% \begin{table}[h]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_with}
% 	\begin{tabular}{c|ccc}
% 		\hline
% 		Width & \tabincell{c}{Memory \\ Footprint (MB)} & FLOPs (M) & \tabincell{c}{Test \\ Accuracy (\%)} \\
% 		\hline
% 		0.25$\times$ & -- & -- & -- \\
% 		0.5$\times$  & -- & -- & -- \\
% 		0.75$\times$ & -- & -- & -- \\
% 		1.0$\times$  & -- & -- & -- \\
% 		\hline
% 	\end{tabular}
% \end{table}
% % To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} propose to prune the global model into a small one.
% % Nevertheless, the pruned parameters cannot be optimized on client's local data, resulting in poor performance.

% % In order to reduce the model complexity without much performance degradation, we decompose the model into two low-rank tensors, named neural basis and coefficient, and only prune the coefficient.
% % The entire neural basis is trained by all clients and the update can be propagated to every model parameter after recomposition, ensuring high model performance.
% % To varify the effectiveness of the proposed approach, we train the models in different complexities (\ie, GPU memory occupancy) over ImageNet-100.
% % The results shown in Fig. \ref{fig:motivation_acc_memory} indicate that the smaller the model, the worse the performance (\ie, accuracy).
% % Besides, it can be observed that the composited model achieves about 5.1\% higher accuracy than the pruned model at the same computing complexity. 

% % There is still one issue when .
% % According to related research, most people use cheap mobile phones with low computing power.
% % Therefore, most clients can only train a small part of coefficient, resulting that the total updating time varies greatly between different coefficient parts.
% % This training inconsistency in updating times may have a negative impact on the convergence performance.
% % We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% % The results in Fig. \ref{fig:motivation_acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% % To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:motivation_acc_hetero}.





% % In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}. 
% % However, the computing capabilities of each clinet may vary significantly and even dynamically in practice \cite{diao2020heterofl}.

% % In practice, the computing capabilities of clients may significantly heterogeneous and even vary dynamically \cite{diao2020heterofl}.

% % In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}, which means a same computational complexity for all clients.
% % Nevertheless, the computing capabilities of clients are generally heterogeneous and may even change dynamically in practice, leading to a long system waiting time in synchronous manner \cite{xu2022adaptive}.
% % Moreover, as the model size continues to increase (\eg, the parameters number of GPT-3 reaches 175 billion \cite{floridi2020gpt}), resource-constrained edge clients may not be able to afford the training overhead (\eg, memory, energy).
% % To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} prune or quantify the global model into a submodel for each client based on its computing capability, so as to alleviate the synchronization barrier issue and diminish the resource consumption.
% % However, for the prune-based methods, the unpruned parameters cannot be optimized in clients' local data, leading to poor performance of global model.
% % Besides, the quantify-based methods will introduce model errors, which also diminishes the performance.
% % Instead of pruning the global model into local ones, FLANC \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% % construct models at various complexities by composing different neural components (\ie, tensors).
% % Instead of pruning or 

% % Different from the above methods, Flanc \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% % The neural basis is trained by all participating clients and the updating can be propagated to every model parameter through neural composition.
% % We trained models in different complexities (\ie, GPU memroy usage) over ImageNet-100 by HeteroFL and Flanc, respectively. 
% % The results shown in Fig. \ref{fig:acc_memory} indicate that the composited model can achieve higher accuracy compared to the pruned model with the same complexity.

% % \begin{figure}[h]
% % 	\centering
% % 	\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}
% % 	\caption{Model performance of different methods.}\label{fig:acc_memory}
% % 	\vspace{-3mm}
% % \end{figure}

% % \begin{figure}[h]
% % 	\centering
% % 	\subfigure[Different computing complexities]{
% % 		\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}\label{fig:motivation_acc_memory}
% % 	}
% % 	\subfigure[Different hetergeneity levels]{
% % 		\includegraphics[width=1.6in]{fig/motivation_acc_hetero.pdf}\label{fig:motivation_acc_hetero}
% % 	}
% % 	\caption{The model accuracy in different conditions.}\label{fig:motivation_model_accuracy}
% % 	\vspace{-3mm}
% % \end{figure}






% \subsection{Impact of local update frequency}
% % Even if FLANC \cite{mei2022resource} enables clients to train complexity-adjustable model.
% % In general, the above techniques are able to custom the model's computing complexity according to clients' computing power.
% % There is still one issue to perform FL in edge computing system.
% % By pruning the coefficient, we can custom the model's computing complexity according to clients' computing power.
% % However, there is still one issue to 
% % However, the edge clients are not only heterogeneous in terms of computing capability, but also in terms of communication capability (\eg, bandwidth) \cite{wang2022accelerating}.
% % As shown in Fig. \ref{fig:round_time_noadloc}, although the local updating time is approximately equal among all clients, the clients with slow communication speed can easily become the bottleneck and lead to long idle time for fast clients. 

% There is still one issue to perform FL in edge computing system.
% Since the clients' capabilities (\eg, computing power, bandwidth) are highly heterogeneous and even time-varying, the stragglers will delay the aggregation and result in long idle time for fast clients.
% As shown in Fig. \ref{fig:round_time_noadloc}, the time cost of the fastest client in one round is only 20\% of the slowest client.
% In other word, 80\% of the fastest client' time is wasted.

% In order to alleviate this problem, we can adjust the numbers of local iterations for different clients, and the effect is illustrated in Fig. \ref{fig:round_time_adloc}.
% On the one hand, the slower can perform fewer local iterations to reduce the impact of stragglers.
% On the other hand, the faster clients can utilize the idle time to perform more local iterations, which helps the model converge faster.
% However, the models trained with different number of local iterations are discrepant, which may affect the convergence performance of global model, especially when the local models' architecture are different.
% Therefore, the existing algorithms to adjust the number of local iterations \cite{wang2018edge} cannot be directly applied in our work. 

% \begin{figure}[h]
% 	\centering
% 	\subfigure[Fixed Updating Frequency]{
% 		\includegraphics[width=1.6in]{fig/motivation_roundtime_noadloc.pdf}\label{fig:round_time_noadloc}
% 	}
% 	\subfigure[Adaptive Updating Frequency]{
% 		\includegraphics[width=1.6in]{fig/motivation_round_adloc.pdf}\label{fig:round_time_adloc}
% 	}
% 	\caption{Ranked clients' time cost in one round.}\label{fig:round_time}
% 	\vspace{-3mm}
% \end{figure}

% % There is still one issue when trianing complexity-adjustable in mobile phones.
% % According to related research, most people use cheap mobile phones with low computing power.
% % Therefore, most client can only train a small part of coefficient, which results that the updating time varies greatly between different clients.
% % This training inconsistency may have a negative impact on the convergence performance.
% % We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% % The results in Fig. \ref{fig:acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% % To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:acc_hetero}.

% However, running these models on edge clients (\eg, smartphones) may encounter performance degradation issues due to the limited computational and communication resources. 

% As the most common terminal device, mobile phones are the primary data source and usually participate in training as clients.
% However, in practice, these phones are generally resource-constrained with poor computing power, so that they may not be able to afford the overhead to train the complete model.

% \begin{table}[t]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_with}
% 	\begin{tabular}{c|ccccc}
% 		\hline
% 		Width & Parameters(M) & Size(MB) & \tabincell{c}{Memory \\ Footprint(MB)} & FLOPs(M) & \tabincell{c}{Test \\ Accuracy(\%)} \\
% 		\hline
% 		0.25$\times$ & -- & -- & -- & -- & -- \\
% 		0.5$\times$  & -- & -- & -- & -- & -- \\
% 		0.75$\times$ & -- & -- & -- & -- & -- \\
% 		1.0$\times$  & -- & -- & -- & -- & -- \\
% 		\hline
% 	\end{tabular}
% \end{table}

% To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} propose to prune the global model into a small one.
% Nevertheless, the pruned parameters cannot be optimized on client's local data, resulting in poor performance.

% In order to reduce the model complexity without much performance degradation, we decompose the model into two low-rank tensors, named neural basis and coefficient, and only prune the coefficient.
% The entire neural basis is trained by all clients and the update can be propagated to every model parameter after recomposition, ensuring high model performance.
% To varify the effectiveness of the proposed approach, we train the models in different complexities (\ie, GPU memory occupancy) over ImageNet-100.
% The results shown in Fig. \ref{fig:motivation_acc_memory} indicate that the smaller the model, the worse the performance (\ie, accuracy).
% Besides, it can be observed that the composited model achieves about 5.1\% higher accuracy than the pruned model at the same computing complexity. 

% There is still one issue when .
% According to related research, most people use cheap mobile phones with low computing power.
% Therefore, most clients can only train a small part of coefficient, resulting that the total updating time varies greatly between different coefficient parts.
% This training inconsistency in updating times may have a negative impact on the convergence performance.
% We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% The results in Fig. \ref{fig:motivation_acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:motivation_acc_hetero}.


% In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}. 
% However, the computing capabilities of each clinet may vary significantly and even dynamically in practice \cite{diao2020heterofl}.

% In practice, the computing capabilities of clients may significantly heterogeneous and even vary dynamically \cite{diao2020heterofl}.

% In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}, which means a same computational complexity for all clients.
% Nevertheless, the computing capabilities of clients are generally heterogeneous and may even change dynamically in practice, leading to a long system waiting time in synchronous manner \cite{xu2022adaptive}.
% Moreover, as the model size continues to increase (\eg, the parameters number of GPT-3 reaches 175 billion \cite{floridi2020gpt}), resource-constrained edge clients may not be able to afford the training overhead (\eg, memory, energy).
% To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} prune or quantify the global model into a submodel for each client based on its computing capability, so as to alleviate the synchronization barrier issue and diminish the resource consumption.
% However, for the prune-based methods, the unpruned parameters cannot be optimized in clients' local data, leading to poor performance of global model.
% Besides, the quantify-based methods will introduce model errors, which also diminishes the performance.
% Instead of pruning the global model into local ones, FLANC \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% construct models at various complexities by composing different neural components (\ie, tensors).
% Instead of pruning or 

% Different from the above methods, Flanc \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% The neural basis is trained by all participating clients and the updating can be propagated to every model parameter through neural composition.
% We trained models in different complexities (\ie, GPU memroy usage) over ImageNet-100 by HeteroFL and Flanc, respectively. 
% The results shown in Fig. \ref{fig:acc_memory} indicate that the composited model can achieve higher accuracy compared to the pruned model with the same complexity.

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}
% 	\caption{Model performance of different methods.}\label{fig:acc_memory}
% 	\vspace{-3mm}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\subfigure[Different computing complexities]{
% 		\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}\label{fig:motivation_acc_memory}
% 	}
% 	\subfigure[Different hetergeneity levels]{
% 		\includegraphics[width=1.6in]{fig/motivation_acc_hetero.pdf}\label{fig:motivation_acc_hetero}
% 	}
% 	\caption{The model accuracy in different conditions.}\label{fig:motivation_model_accuracy}
% 	\vspace{-3mm}
% \end{figure}

% Even if FLANC \cite{mei2022resource} enables clients to train complexity-adjustable model.
% In general, the above techniques are able to custom the model's computing complexity according to clients' computing power.
% There is still one issue to perform FL in edge computing system.
% By pruning the coefficient, we can custom the model's computing complexity according to clients' computing power.
% However, there is still one issue to 
% However, the edge clients are not only heterogeneous in terms of computing capability, but also in terms of communication capability (\eg, bandwidth) \cite{wang2022accelerating}.
% As shown in Fig. \ref{fig:round_time_noadloc}, although the local updating time is approximately equal among all clients, the clients with slow communication speed can easily become the bottleneck and lead to long idle time for fast clients. 
% There is still one issue to perform FL in edge computing system.
% Since the clients' capabilities (\eg, computing power, bandwidth) are highly heterogeneous and even time-varying, 

% As shown in Fig. \ref{fig:round_time_noadloc}, the time cost of the fastest client in one round is only 20\% of the slowest client.

% There is still one issue when trianing complexity-adjustable in mobile phones.
% According to related research, most people use cheap mobile phones with low computing power.
% Therefore, most client can only train a small part of coefficient, which results that the updating time varies greatly between different clients.
% This training inconsistency may have a negative impact on the convergence performance.
% We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% The results in Fig. \ref{fig:acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:acc_hetero}.

% Moreover, the heterogeneity among the clients, \ie, the computing power and communication capacity of different edge clients is significantly varied, will also have a great impact on training efficiency.
% For example, the hardware manufacturer typically configure 
% For example, mobile manufacturers typically configure multiple processors (\eg, Snapdragon, Apple A-series chips) on the client to cater to the diverse needs of customers, however, resulting in inconsistent completion time for model training.
% Besides, the computing power and communication capacity of different edge clients is significantly varied, which will have a great impact on training efficiency.
% For example, there can be a tenfold difference in CPU frequency or bandwidth for the edge devices \cite{xu2022adaptive}.
% In synchronous mode, clients with faster training and/or communication speed often have to wait the stragglers for global aggregation, resulting in a longer or even unacceptable completion time of model training.
% In addition, due to the intrinsic and/or external conditions, such as ambient temperatures, CPU states,
% network connections to the server and so on, the per-round computing time and communication time at each client may vary significantly.
% The different network connection methods (\eg, 4G, 5G and WIFI) of the client also affect the communication cost of model transmission during the training process\cite{}.
% Besides, the availability and connectivity of edge clients may change over time, \ie, network dynamics.
% For instance, the smartphone can freely join or exit the training process. 
% The addition of clients will increase the scale and data diversity of training, while the withdrawal of clients may lead to data loss during training, leading to the performance degradation of the model training.

% Moreover, the heterogeneity among the clients, \ie, the computing power and communication capacity of different edge clients is significantly varied, will also have a great impact on training efficiency.
% For example, the hardware manufacturer typically configure 
% For example, mobile manufacturers typically configure multiple processors (\eg, Snapdragon, Apple A-series chips) on the client to cater to the diverse needs of customers, however, resulting in inconsistent completion time for model training.

% The different network connection methods (\eg, 4G, 5G and WIFI) of the client also affect the communication cost of model transmission during the training process\cite{}.
% Besides, the availability and connectivity of edge clients may change over time, \ie, network dynamics.
% For instance, the smartphone can freely join or exit the training process. 
% The addition of clients will increase the scale and data diversity of training, while the withdrawal of clients may lead to data loss during training, leading to the performance degradation of the model training.

% For example, performing one mini-batch SGD on standard ResNet-18\footnote{Image resolution is 3$\times$144$\times$144, batch size is 32.} with NVIDIA Jetson TX2\footnote{A commercial edge embedded AI computing device. More details are available at https://www.nvidia.cn/autonomous-machines/embedded-systems} takes xxx minutes and consumes xx\% of the battery.


% Different from pruning the global model directly, \textit{Flanc} \cite{mei2022resource} proposes to construct the models in different width by multiplying the neural basis with different coefficient.
% The neural basis is shared by all clients, which enables every parameter in global model to access the full range of knowledge of all clients, improving the performance of global model.
% Despite the improvement, \textit{Flanc} only aggregates the coefficients with the same shape, thus the learned coefficient will be biased towards the data distribution of corresponding particular clients set, which hurts the generalization performance of the global model when the local datasets are Non-IID.
% To verify this phenomenon, we test the \textit{HeteroFL} and \textit{Flanc} by training CNN on CIFAR-10 under three different Non-IID levels, denoted by \textit{low}, \textit{medium} and \textit{high}, respectively. 
% The results shown in Table \ref{table:motivation_training_heterogeneous_models} indicate that \textit{Flanc} achieves better performance than \textit{HeteroFL}, but the test accuracies of both \textit{Flanc} and \textit{HeteroFL} are significantly decreased as the Non-IID level increases.
% To this end, we design a novel neural composition technique to aggregate the coefficients in different shape into a global one and let the parameter in global coefficient be evenly trained, so as to improve the training robustness against Non-IID data.
% By Table \ref{table:motivation_training_heterogeneous_models}, the global model can achieve the best test accuracy with our proposed technique. 


% Therefore, it is necessary to reduce the model complexity for these resource-constrained clients by reducing the model's depth (\ie, number of layers) \cite{kim2023depthfl} or width (\ie, number of hidden channels) \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex}.
% In this work, we mainly focus on adjusting the model complexity by modulating the model width, which can reduce parameters and memory footprint during raining more effectively compared to reducing model depth \cite{mei2022resource}.

% Some techniques (\eg, model pruning) can significantly reduce the computing complexities and training overhead of a DNN model, but it usually comes with performance degradation.
% Reducing the model width can significantly reduce the computing complexities and training overhead, but it usually comes with performance degradation.
% To evaluate the impact of model width on FL training, we construct a CNN model with three 3$\times$3 convolutional layers and one fully-connected layer, where each convolutional layer has 64, 128 and 128 hidden channels, respectively.
% We reduce the model width by 0.25, 0.5, 0.75 and 1.0 times, and record the model's training overhead and test accuracy over CIFAR-10, respectively.
% The results in Table. \ref{table:motivation_models_in_different_width} indicate that the smaller the model width, the less training overhead, but the lower the accuracy.
% For instance, the 1.0-width model needs about 15 times more FLOPs to process an image than the 0.25-width model, but its test accuracy is 6.29\% higher.
% To minimize the performance degradation, the model width should be as large as possible within the clients' computing power.

% \begin{table}[t]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_width}
% 	\begin{tabular}{c|cccc}
% 		\hline
% 		Width & 0.25$\times$ & 0.5$\times$ & 0.75$\times$ & 1.0$\times$ \\
% 		\hline
% 		Parameters(K) & 34.87 & 97.29 & 187.4 & 305.16 \\
% 		Size(MB) & 0.13 & 0.37 & 0.72 & 1.16 \\
% 		Memory Footprint(MB) & 22.35 & 59.64 & 68.69 & 92.16 \\
% 		FLOPs(M) & 7.68 & 29.52 & 65.51 & 115.65 \\
% 		Test Accuracy(\%) &  81.09 & 85.05 & 86.65 & 87.38 \\
% 		\hline
% 	\end{tabular}
% \end{table}

% In FL, each client performs model training on its local dataset and then sends the updated model to the parameter server (PS). 
% Once receiving the local updated models from clients, PS will aggregate them and distribute the fresh global model to the clients for the next round of training. 
% The whole process continues until the global model converges.
% As the field continues to evolve, FL holds significant potential for advancing the capabilities of edge computing and enabling intelligent applications in diverse domains, such as healthcare, autonomous vehicles, and smart cities \cite{rahman2021challenges}.

% Despite the advantages of FL, the growing complexity (\eg, the parameter size or architecture) of deep neural networks (DNNs) incurs a large amount of computation and communication overhead during model training.
% Computation and Communication Resource Limitation.
% Mobile Phones cannot train the DNNs models
% iPhone....

% In order to reduce the communication cost, some existing works \cite{hsieh2017gaia} propose to perform multiple local updates on the clients before uploading the models or gradients to the PS for aggregation. However, setting the same local update frequency for each client will lead to the problem of synchronization barriers in heterogeneous systems, \ie, the stragglers (\ie, weak clients) will delay the aggregation and result in long idle time for the strong clients.


% Related Works:
% 1) Local Update Frequency Optimization
% 2) Gradient Compression
% 3) Model Pruning

% Introduce Neural Composition

% Nevertheless, the system heterogeneity is still a challenge

% We propose a novel framework to ....
% Firstly, the computation resource is always constrained on edge clients, such as smartphones and Internet of Things (IoT) devices.
% For example, the floating-point operations per second (FLOPS) of an iPhone14 is 18.2$\times$ smaller than that of desktop GPU RTX3090.

% Different from data centers where the server clusters communicate with each other over high-speed LANs, edge clients usually communicate with PS through WANs, whose bandwidth is much lower than that of LANs.

% Consequently, the frequent model transmissions will result in a long communication time, potentially becoming a bottleneck in the training process.
% On the other hand, 
% For instance, a standard ResNet-18 \cite{he2016deep} consists of 11.68 million parameters and requires 27.29 billion floating-point operations (FLOPs) to classify a single image, making the local update process extremely slow or even infeasible on edge clients \cite{jiang2022fedmp}.


% For example, smartphones are an important data source, yet their computation resource is severely limited (\eg, CPU power, RAM, battery).
% To perform efficient model training over the weak clients like smartphones, \textit{HeteroFL} \cite{diao2020heterofl} prunes 93.75\% of the parameters from the complete model.
% In other words, only 6.25\% of the parameters are optimized while the majority of the parameters can not benefit from the smartphones' local data, leading to poor training performance of the complete model.

% Nevertheless, pruning restricts the clients' contributions to only a small portion of the global model, resulting in under-optimized pruned parameters and significant performance degradation.
% For example, 

% However, \textit{Flanc} only aggregates coefficients with the same shape, which will introduce the training bias towards specific client sets. 
% This limitation negatively impacts the generalization performance of the global model, particularly when dealing with non-independent and non-identically distributed (Non-IID) local datasets.

%and making the training process inefficient.
% However, the upload speed of this client is very slow, which will lead to long completion time, delay the aggregation step and make the training process inefficient.
% In synchronous mode, clients with fast computation and/or communication speed often have to wait for the stragglers for global aggregation, resulting in a longer or even unacceptable completion time.
% For example, due to the expensive price, the high-performance clients are typically rare in the edge system.
% The largest coefficient can only benefit from a few powerful clients, thus the largest global model may not convergence within the given completion time, leading to poor training performance.

% 1) \textit{Limited Computation Resource.}
% The 
% For example, the standard ResNet-18 \cite{he2016deep} contains 11.68 million parameters and requires 27.29 billion floating-point operations (FLOPs) to classify a single image, making the local update process extremely slow or even infeasible on edge clients \cite{jiang2022fedmp}.
% 2) \textit{Limited Communication Resource.}
% Besides, the bandwidth of wide area networks (WANs) between the parameter server (PS) and edge clients is much (\eg, 15$\times$) lower than that of local area networks (LANs) within the data centers \cite{wang2021resource}. 
% Consequently, the frequent model transmissions will result in a long communication time, potentially becoming a bottleneck in the training process.
% 3) \textit{Client Heterogeneity.}
% Moreover, the computing power and communication capacity of different edge clients is significantly varied.
% For example, there can be a tenfold difference in CPU frequency or bandwidth for the edge clients \cite{xu2022adaptive}.
% In synchronous mode, clients with fat computation and/or communication speed often have to wait for the stragglers for global aggregation, resulting in a longer or even unacceptable completion time.

% Despite the advantages of FL, the growing complexity (\eg, the parameter size or architecture) of deep neural networks (DNNs) incurs a large amount of computation and communication overhead during model training.
% For example, the standard ResNet-18 \cite{he2016deep} contains 11.68 million parameters and requires 27.29 billion floating-point operations (FLOPs) to classify a single image, making the local update process extremely slow or even impossible on the resource-constrained edge clients \cite{jiang2022fedmp}.
% Besides, the bandwidth of wide area networks (WANs) between the parameter server (PS) and edge clients is much (\eg, 15$\times$) lower than that of local area networks (LANs) within the data centers \cite{wang2021resource}. 
% Consequently, the frequent model transmissions will result in a long communication time, potentially becoming a bottleneck in the training process.




% In order to simultaneously save the computation and communication resources in FL, a natural solution is to prune the global model into the smaller sub-models according to the clients' resource constraints \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl}.
% For example, \textit{HeteroFL} \cite{diao2020heterofl} prunes excessive hidden channels in each layer, while \textit{DepthFL} \cite{kim2023depthfl} prunes the deepest layers from the global model.
% Nevertheless, pruning restricts the clients' contributions to only a small portion of the global model, resulting in under-optimized pruned parameters and significant performance degradation.

% To address this issue, \textit{Flanc} \cite{mei2022resource} proposes to approximate the deep learning model as the product of two low-rank tensors, named neural basis and coefficient.
% The model at different widths can be constructed by composing (\ie, multiplying) the neural basis with coefficients of different shapes.
% The entire neural basis is trained by all clients and its update can be propagated to every parameter of the global model through composition, allowing the full global model to benefit from the knowledge of all clients.
% However, \textit{Flanc} only aggregates coefficients with the same shape, which will introduce the training bias towards specific client sets. 
% This limitation negatively impacts the generalization performance of the global model, particularly when dealing with non-independent and non-identically distributed (Non-IID) local datasets.
% However, \textit{Flanc} only aggregates the coefficients with the same shape and the learned coefficient will be biased towards the corresponding particular clients set, which hurts the generalization performance of the global model especially when the local datasets are not independent and identically distributed (Non-IID).
% To eliminate the training deviation of coefficients, we propose to adopt a novel neural composition technique that aggregates the coefficients with different shapes into a global one, enabling every parameter in the global model to be fully trained.


% In this way, the entire neural basis is trained by all clients and its obtained update can be propagated to every parameter of the global model through composition. 
% However, \textit{Flanc} only aggregates the coefficients with the same shape, which makes the learned coefficient biased towards the corresponding particular group of clients. 
% However, the computing power and communication capacity of different edge clients is significantly varied, which will have a great impact on training efficiency.
% Despite reducing model complexity to save computing and communication resources through neural composition,
% Despite the resource saving by neural composition technique,
% In addition to the resource limitation, FL also faces two critical challenges, \ie, client heterogeneity and dynamics, which will have a great impact on training efficiency.
% Firstly, the computing power and communication capacity of different edge clients is significantly varied.
% For example, there can be a tenfold difference in CPU frequency or bandwidth for the edge clients \cite{xu2022adaptive}.
% Besides, due to the dynamic of network condition and the instability of clients states, the per-round computing time and communication time at each client may also vary significantly.
% In synchronous mode, clients with fast training and/or communication speed often have to wait for the stragglers for global aggregation, resulting in a longer or even unacceptable completion time of model training.



% In order to synchronize the training process of heterogeneous clients in a dynamic environment, some works propose to control each participating client's computing time \cite{li2020federated, xu2022adaptive, li2022pyramidfl} or communication time \cite{li2021talk, cui2022optimal, jiang2022adaptive}.
% For example, \textit{FedProx} \cite{li2020federated} adaptively determines proper local update frequency for each participating client based on its constrained resource, so as to balance the computing time of different clients.
% \textit{FlexCom} \cite{li2021talk} adopts the model compression technique (\eg, quantization or sparsification) to alleviate the communication load and dynamically adjusts the compression ratio for each participating client on the basis of time-varying link speed, thus balancing the communication time across different clients.
% However, all of these schemes require the participating clients to train the complete model, which will strain the limited computation resources available on edge clients.

% \begin{table}[t]
% \centering
% \setlength{\abovecaptionskip}{10pt}%
% \setlength{\belowcaptionskip}{0pt}%
% \footnotesize
% \caption{Comparison of different FL schemes.}
% \label{table:FL_schemes_comparison}
% \begin{tabular}{c|c|c|c}
% \hline
% FL schemes & \tabincell{c}{Resource \\ Efficiency} & \tabincell{c}{Heterogeneity \\ and Dynamic} & \tabincell{c}{Performance \\ 
% Guarantee}\\
% \hline
% \tabincell{c}{Model \\ Pruning } \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex} & \checkmark & \ding{55} & \ding{55} \\
% \hline    
% \tabincell{c}{Gradient \\ Compression} \cite{li2021talk, cui2022optimal, jiang2022adaptive} & \ding{55} & \checkmark & \ding{55}  \\
% \hline
% \tabincell{c}{Frequency \\ Optimization} \cite{li2020federated, xu2022adaptive, li2022pyramidfl}  & \ding{55} & \checkmark & \checkmark\\
% \hline
% \tabincell{c}{\textbf{Proposed} \\ \textbf{Framework}}  & \checkmark & \checkmark & \checkmark \\
% \hline
% \end{tabular}
% \end{table}


% As summarized in Table \ref{table:FL_schemes_comparison}, the existing works cannot fully address the challenges of resource limitation, client heterogeneity and dynamics with the performance guarantee.
% To this end, we propose a novel FL framework, named Heroes, which investigates the benefits of neural composition technique and adaptive local update frequency so as to reduce the resource cost and eliminate the idle time incurred by synchronization.
% However, the neural composition and local update frequency are coupled. 
% Concretely, the completion time depends on the size of composed model, which affects the determination of local update frequency.
% Meanwhile, the local update frequency also affects the training adequacy of each parameter.
% Therefore, \textit{it is necessary yet challenging to jointly assign proper coefficient blocks and determine the optimal local update frequency for each client.}
% Our contributions are summarized as follows:
% Concretely, we modify the model width by controlling the size of coefficient tensor for each client based on its computing power to save both the limited computing and communication resources.
% Additionally, we adjust the local update frequencies for heterogeneous clients to balance their completion time and let the parameters in coefficient tensor be evenly trained.
% \textit{Nevertheless, how to assign appropriate coefficient and local update frequencies to heterogeneous clients remains an important challenge in Heroes.}
% \begin{itemize}
%     \item We propose a novel FL framework, called Heroes, which overcomes the challenges of resource limitation as well as client heterogeneity and dynamic by adaptive neural composition and local update.
%     \item We theoretically analyzed the convergence of Heroes and formulated the optimization problem. Guided by the convergence bound, we propose a control algorithm to adjust the coefficient tensor and determine the local update frequency for each participating client.
%     \item The experimental results demonstrate that Heroes can speedup the training process by up to 2.4$\times$ and improve the test accuracy by about 8.75\% compared with the baselines.
    % \item We conduct extensive experiments on typical models and real-world datasets to show the effectiveness and efficiency of our proposed framework. The experimental results demonstrate that Heroes can speedup the training process by up to 2.4$\times$ and improve the test accuracy by about 8.75\% compared with the baselines.
% \end{itemize}

% The rest of this paper is organized as follows. 
% Section \ref{sec:motivation} introduces the background and motivation for our work.
% Section \ref{sec:prelim} states the process of the proposed framework.
% Section \ref{sec:analysis} provides the convergence analysis of xxx.
% Section \ref{sec:algorithm} formulates the optimization problem and designs the control algorithm.
% Section \ref{sec:evaluation} presents the evaluation results.
% Section \ref{sec:related} reviews related work and we conclude this paper in Section \ref{sec:conclusion}.
% \textit{FedAvg} \cite{mcmahan2017communication} is the pioneer and also the most widely used FL method to solve the problem in Eq. \eqref{eq:fl_goal}.

% Let $\mathbf{x}^{h}$ denote the global model in round $h$. 
% Generally, complex models (\eg, deeper architecture or more number of parameters) tend to provide better training performance because they have stronger expressive power \cite{zhang2021understanding}. 
% However, training these models will consume excessive computational and communication resources, leading to long completion time or even inability to run on edge clients.

% According to the low-rank decomposition techniques, $\mathbf{w}$ can be approximated as $\mathbf{w} \approx \mathbf{v} \cdot \mathbf{u}$, where $\mathbf{v} \in \mathbb{R}^{k^{2} \times PI \times R}$ and $\mathbf{u} \in \mathbb{R}^{R \times PO}$.
% It means that we can obtain the models in different widths by adjusting the shape of $\mathbf{v}$ or $\mathbf{u}$.
% Thus, the model' width is related to the shape of $\mathbf{v}$ or $\mathbf{u}$.
% Suppose that we reduce the model width by up to $P$ times, 
% Based on the low-rank decomposition technique \cite{phan2020stable}, ]
% The weights in different widths only differ on the shape of coefficient while the shape of basis is constant.
% The weight's width depends on the shape of coefficient, and the shape of basis is constant.
% Thus, we reduce the model width by only reducing the size of coefficient $\mathbf{u}$.
% Thus, we can control the weight's width by adjusting the coefficient.
% Thus, the weight's width can be controlled by adjusting the size of coefficient.

% We select $p^{2}$ parts of coefficient to composite with neural basis to obtain the $p$-width model.

% We measure the amount of training each block has obtained by the total local iterations it has experienced on all clients since round 1, \ie, total update times.
% For the convenience of expression, we utilize $c_{i}^{h}$ to represent the total update times of block $i$ in round $h$.
% Notably, to ensure the sufficient training for all coefficient blocks, the selected $p^{2}$ blocks are the ones with the least training.
% Instead of pruning model parameters directly, 
% Compared to the prune-based schemes, where the pruned model parts cannot be optimized, this approach can improve the training stability and performance, beacuse the entire neural basis $\mathbf{v}$ get update over all clients' local data (\ie, learn knowledge from all clients) and the update can be propagated to every model parameter through composition.

==> fig/content/abstract.tex <==
Federated Learning (FL) enables distributed clients to collaboratively train models without exposing their private data.
However, it is difficult to implement efficient FL due to limited resources.
Most existing works compress the transmitted gradients or prune the global model to reduce the resource cost, but leave the compressed or pruned parameters under-optimized, which degrades the training performance.
To address this issue, the neural composition technique constructs size-adjustable models by composing low-rank tensors, allowing every parameter in the global model to learn the knowledge from all clients. 
Nevertheless, some tensors can only be optimized by a small fraction of clients, thus the global model may get insufficient training, leading to a long completion time, especially in heterogeneous edge scenarios.
To this end, we enhance the neural composition technique, enabling all parameters to be fully trained.
Further, we propose a lightweight FL framework, called Heroes, 
with enhanced neural composition and adaptive local update.
A greedy-based algorithm is designed to adaptively assign the proper tensors and local update frequencies for participating clients according to their heterogeneous capabilities and resource budgets.
Extensive experiments demonstrate that Heroes can reduce traffic consumption by about 72.05\% and provide up to 2.97$\times$ speedup compared to the baselines.

% access the full range of knowledge.
% To address this issue, neural composition technique approximates the model as the product of two low-rank tensors, allowing every parameter access the full range of knowledge.
% thus the global model may get insufficient training, leading to long completion time, especially in the heterogeneous network.
% 
% Different from compression and pruning, neural composition technique constructs the models at various complexities by multiplying tensors of different sizes.
% allowing every parameter access the full range of knowledge.
% Nevertheless, tensors of different sizes are aggregated independently, which disperses the clients' contribution and slows down the convergence of global model.
% Nevertheless, the global models composed of different tensors are often unevenly trained, leading to slow convergence speed, especially in heterogeneous edge clients.

% Neural composition technique constructs the models at various complexities by multiplying two low-rank tensors, allowing every parameter learn the knowledge from all clients.


% Based on the enhanced neural composition, we propose a novel and lightweight FL framework, called Heroes, to overcome the challenges of resource limitation and client heterogeneity while maintaining the training performance of original model with fast convergence speed.


% Federated Learning (FL) enables collaborative model training across distributed edge clients, which protects the users' privacy. 
% However, it is difficult to implement efficient FL over the practical edge network due to the limited computation and communication resources.
% To this end, a natural solution is to prune the global model into a smaller sub-model, where the pruned parameters cannot benefit from the clients' local data, leading to poor training performance.
% Neural composition technique constructs the models in different complexities by composing two low-rank tensors, enabling every parameter to learn the knowledge from all clients.
% Nevertheless, the global model may get insufficient training, leading to slow convergence speed.
% Besides, the client heterogeneity also hurts the training efficiency significantly.
% To tackle these issues, we propose a novel and lightweight FL framework, named Heroes, with an enhanced neural composition technique and adaptive local update, to overcome the challenges of resource limitation and client heterogeneity while maintaining the accuracy of global model.
% Extensive experiments demonstrate that Heroes can reduce traffic consumption by about 72.05\% and provide up to 2.97$\times$ speedup for the training process compared to the baselines.

%named neural basis and coefficient.
% Models at various complexities are constructed for different clients by composing neural basis with coefficients of different sizes.
% This approach allows every parameter in the global model access the full range of knowledge, by training neural basis on all clients.
% Nevertheless, the coefficients are aggregated separately according to their different sizes, thus there are several global models and each global model may get insufficient training, leading to slow convergence speed.
% Besides, the stragglers also hurts training efficiency greatly due to the client heterogeneity.



% In practice, deep learning models tend to become more complex (\eg, more number of parameters),u bringing several benefits, such as higher accuracy and feature representation.
% Intuitively, the increasingly complex models (\eg, more number of parameters) can improve the training performance.
% Nevertheless, the limited computation and communication resources will significantly degrade the training performance.
% To address the above issues, a natural solution is to reduce the model complexity (\eg, pruning). 
% However, the different portions of the model will be unevenly trained over the local data, resulting in under-optimized pruned parameters, especially in heterogeneous edge networks. 
% Neural composition decomposes the model into two lighter tensors to reduce resource costs, while ensuring that all parameters are evenly trained. 
% To this end, we propose a novel FL framework, named Heroes, with an enhanced neural composition technique for efficient FL training.
% Meanwhile, Heroes adaptively assigns different local update frequencies to the heterogeneous clients, significantly eliminating the idle time incurred by synchronization and accelerating the model training process.
% The experimental results demonstrate that compared to the baselines, Heroes can reduce the traffic consumption by about 62.5\% and provide by up to 1.7$\times$ speedup for the training process while achieving the same accuracy on the real-world datasets.
% the computing and communication resources available on edge clients are always  limited, resulting in significant performance degradation. 


==> fig/content/algorithm.tex <==
% In this section, we first define the optimization problem of our proposed framework.
% Then, we propose an update algorithm that dynamically determines the model width and the local update frequencies for different clients.
% We first present the preliminaries for our algorithm design and then introduce the proposed algorithm in detail.

\subsection{Problem Formulation}

% In this section, we define the problem of efficient FL with adaptive neural composition and local updating. 
In this section, we define the joint optimization problem of neural composition and local update frequency in FL training.
Let $G(\mathbf{v} \cdot \mathbf{u})$ represent the number of floating-point operations (FLOPs) required to perform one local iteration for the composed model, and $G(\mathbf{v} \cdot \mathbf{u})$ depends on the size of coefficient $\mathbf{u}$.
The more blocks the coefficient $\mathbf{u}$ includes, the wider the composed model $\mathbf{x} = \mathbf{v} \cdot \mathbf{u}$ and the more FLOPs required for model training.  
We formulate the time cost for one local iteration of client $n$ in round $h$ as follows:
% \vspace{-3mm}

\begin{equation}
    \mu_{n}^{h} = G(\mathbf{v}^{h}_{n} \cdot \hat{\mathbf{u}}^{h}_{n}) / q_{n}^{h}
\end{equation}
where $q_{n}^{h}$ represents the speed to process the floating-operations of client $n$ in round $h$.

Since the download bandwidth is usually much faster than the upload bandwidth in typical WANs \cite{zhan2020incentive}, the download time of tensors can be negligible and we mainly focus on the upload time. 
% The upload bandwidth of client $i$ at round $k$ is represented by $b_{i}^{k}$. Let $h(V)$ and $h(U^{k}_{p_{i}})$ denote the size of basis and coefficient, respectively. 
Let $b_{n}^{h}$ denote the upload bandwidth of client $n$ in round $h$ and $E$ measure the size of a tensor.
We formulate the communication time of client $n$ in round $h$ as:
\begin{equation}
    \nu_{n}^{h} = [E(\bar{\mathbf{v}}_{n}^{h}) + E(\bar{\mathbf{u}}_{n}^{h})] / b_{n}^{h}
\end{equation}
% where $\bar{\mathbf{v}}_{n}^{h}$ and $\bar{\mathbf{u}}_{n}^{h}$ represent the neural basis and coefficient updated by client $n$ in round $h$, respectively.

% In general, the time cost of client $n$ in round $h$ includes $t_{i}^{k, cp}$ for local updating and $t_{i}^{k, cm}$ for communication with PS, \ie, $t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}$. 
Let $T_{n}^{h}$ denote the completion time of client $n$ in round $h$, which consists of the time cost for $\tau_{n}^{h}$ local iterations and the communication time.
Due to the synchronization barrier of FL, the completion time of round $h$ depends on the slowest client, which can be defined as:
\begin{equation}
    T^{h} = \mathop{\max}_{n \in \mathcal{N}^{h}}  T_{n}^{h} = \mathop{\max}_{n \in \mathcal{N}^{h}} (\tau_{n}^{h} \cdot \mu_{n}^{h} + \nu_{n}^{h}) 
\end{equation}

We adopt the average waiting time for participating clients in $\mathcal{N}^{h}$ to measure the impact of synchronization barrier in round $h$, which is defined as follows:
\begin{equation}
    \mathcal{W}^{h} = \frac{1}{K} \sum_{n \in \mathcal{N}^{h}} (T^{h} - T_{n}^{h})
\end{equation}

Let $c_{i}^{h}$ denote the total update times of $i$-th coefficient block, where $i \in \{1, 2, \cdots, P^{2} \}$.
The training consistency between different coefficient blocks in round $h$ can be reflected by the variance of set $\{ c_{i}^{h} | \forall i\}$, denoted as:
\begin{equation}
    \mathcal{V}^{h} = \frac{1}{P^{2}} \sum_{i=1}^{P^{2}} ( c_{i}^{h} - \frac{1}{P^{2}} \sum_{j=1}^{P^{2}} c_{j}^{h})^{2}
\end{equation}





% In each round $k$, we aim to choose an appropriate coefficient $U^{k}_{p_{i}}$ for each participating client $i$ based on its computation capability, and determine the optimal number of local iterations $\tau_{i}^{k}$, so as to accelerate the training process of FL. We define the optimization problem as follows:

In each round $h$, we aim to select appropriate $(p_{n}^{h})^{2}$ coefficient blocks and determine the optimal local update frequency $\tau_{n}^{h}$ for each participating client $n \in \mathcal{N}^{h}$, so as to accelerate the training process of FL.
Accordingly, we define the optimization problem as follows:

\centerline{$\mathop{\min} \sum_{h=1}^{H} T^{h}$}
\begin{equation} \label{eq:problem_formulation}
    s.t.
    \begin{cases} 
    F(\mathbf{v}^{H} \cdot \mathbf{u}^{H}) \leq \epsilon  \\
    \mathcal{W}^{h} \leq \rho, & \forall h \\
    \mathcal{V}^{h} \leq \delta, & \forall h \\
    p_{n}^{h} \in \{ 1, 2, \cdots, P \}, & \forall n, h
    \end{cases} 
\end{equation}

The first inequality expresses the convergence requirement, where $\epsilon$ is the convergence threshold of the training loss after $H$ rounds. 
The second set of inequalities indicates that the average waiting time of participating clients in each round $h$ should not exceed the given threshold $\rho$.
The third set of inequalities bounds the variance of all coefficient blocks' total update times in each round $h$, ensuring the balanced training among blocks. 
% ensures even training among different coefficient blocks, where the variance of all blocks' total update times is bounded by threshold $\delta$ in each round $h$.
The fourth set of inequalities tells the feasible range of the number of coefficient blocks.
The object of this optimization problem is to minimize the completion time of the FL training with the performance requirements (\eg, model convergence, average waiting time).


\begin{algorithm}[t]
	\caption{ Procedure at the PS} \label{alg:ps}
    \algnotext{EndFor}
    \algnotext{EndWhile}
    \algnotext{EndIf}
    \algnotext{label}
	\algorithmicrequire{ completion time budget $T^{max}$, maximum time cost for one local iteration $\mu^{max}$, maximum model width $P$, waiting time bound $\rho$.}\\
	\algorithmicensure{ convergenced neural basis $\mathbf{v}^{H}$ and coefficient $\mathbf{u}^{H}$.}
	\begin{algorithmic}[1]
		\State Initialize $\mathbf{v}^{0}$ and $\mathbf{u}^{0}$ as random tensors;
        \State Initialize $h \leftarrow 0$, $T \leftarrow 0$, $c_{i}^{h} \leftarrow 0$ ($\forall i \in [P^{2}]) $;
		\While { $T \leq T^{max}$ }
        \State Collect the status information of network and clients;
        \State Randomly sample $K$ participating clients, \ie, $\mathcal{N}^{h}$;
        % \State Split coefficient $\mathbf{u}^{h}$ into $P$ parts $\{\mathbf{i}^{h}_{p} | p \in [P] \}$;
		\For {each client $n \in  \mathcal{N}^{h}$}
  \label{alg:ps_determine_block_number_begin}
        % \State Set $\mu_{n}^{h} \leftarrow 0$, $I_{n}^{h} \leftarrow 1$, $\hat{\mathbf{u}}^{h}_{n} \leftarrow NULL$; 
        % \State Set $\mathcal{C} \leftarrow \{C_{p} | p \in [P] \}$, $\mathcal{O}_{n}^{h} \leftarrow \emptyset$; 
        \State Set $\mu_{n}^{h} \leftarrow 0$ and $p_{n}^{h} \leftarrow 1$; 
        \While{$\mu_{n}^{h} < \mu^{max}$ and $p_{n}^{h} < P$}
        % \State $\hat{\mathbf{u}}^{h}_{n} \leftarrow $ concate $ \mathbf{i}^{0}_{1}$ for $p_{n}^{h}$ times;
        % \State $o \leftarrow \mathop{\arg\min}_{p} C_{p}$;
        % \State $\mathcal{C} \leftarrow \mathcal{C} - \{C_{o}\} $, $\mathcal{O}_{n}^{h} \leftarrow \mathcal{O}_{n}^{h} + \{ o\}$;
        % \State  Concate $\hat{\mathbf{u}}^{h}_{n}$ with $\mathbf{i}_{o}^{h}$ and $\hat{\mathbf{x}}^{h}_{n} \leftarrow \mathbf{v}^{h} \cdot \hat{\mathbf{u}}^{h}_{n}$;
        % \State Add a block into coefficient;
        \State Estimate the local iteration time $\mu_{n}^{h}$;
        \State Set $p_{n}^{h} \leftarrow p_{n}^{h} + 1$;
        \EndWhile
        \State Estimate the communication time $\nu_{n}^{h}$; \label{alg:ps_determine_block_number_end}
		\EndFor
		% \State Minimize $T(H, \tau) = (H-h) \cdot (\tau \cdot \mu_{n}^{h} + \nu_{n}^{h})$;
        % \State Obtain $T_{n}$ and $\tau_{n}$;
        \For { each client $n \in  \mathcal{N}^{h}$} \label{alg:ps_select_l_begin}
        \State Solve Eq. \eqref{eq:approximated_client_n_completion_time} to obtain $T_{n}$, $\tau_{n}$ and $T_{n}^{h}$; 
        \EndFor 
        \State Select the fastest client $l \leftarrow \mathop{\arg\min}_{n \in \mathcal{N}^{h}} T_{n}$; \label{alg:ps_select_l_end}
        \State Set $\tau_{l}^{h} \leftarrow \tau_{l}$ and $T \leftarrow T + T_{l}^{h}$;\label{alg:ps_determine_other_tau_begin}
        \For { each client $n \in  \mathcal{N}^{h}$} 
        \If {$n \neq l$}
        \State Obtain the interval $[\tau_{a}, \tau_{b}]$ by Eq. \eqref{eq:approximate_waiting_time};  
        \State Search $\tau_{n}^{h} \in [\tau_{a}, \tau_{b}]$ to minimize $\mathcal{V}^{h}$; \label{alg:ps_determine_other_tau_end}
        \EndIf
        \State Select the least trained $(p_{n}^{h})^{2}$ blocks to form $\hat{\mathbf{u}}^{h}_{n}$;
        % \State Update $c_{i}^{h} (\forall i \in [P^{2}])$;
        \For {each coefficient block $i$ in $\hat{\mathbf{u}}_{n}^{h}$ }
        \State Update $c_{i}^{h} \leftarrow c_{i}^{h} + \tau_{n}^{h}$;
        \EndFor
        % \For { block $p$ in $\hat{\mathbf{u}}^{h}_{n}$}
        % \State $c_{p} \leftarrow c_{p} + \tau_{n}^{h}$;
        % \EndFor 
        \State Send $\mathbf{v}^{h}$, $\hat{\mathbf{u}}_{n}^{h}$, $\tau^{h}_{n}$ to client $n$;
		\State Receive $L_{n}$, $\sigma_{n}^{2}$, $G_{n}^{2}$, $\bar{\mathbf{v}}^{h}_{n}$, $\bar{\mathbf{u}}_{n}^{h}$ from client $v_{n}$;
        \EndFor 
        % \State Aggregate the estimated variables: $L \leftarrow \frac{1}{K} \sum_{n \in \mathcal{N}^{h}} L_{n}$, $\sigma^{2} \leftarrow \frac{1}{K} \sum_{n \in \mathcal{N}^{h}} \sigma^{2}$ and $G^{2} \leftarrow \frac{1}{K} \sum_{n \in \mathcal{N}^{h}} G^{2}$; 
        \State Aggregate estimated variables to $L$, $\sigma^{2}$ and $G^{2}$; 
        \label{alg:ps_global_aggregation_begin}
        % \State $\sigma^{2} \leftarrow \frac{1}{K} \sum_{n \in \mathcal{N}^{h}} \sigma^{2}$;
        % \State $G^{2} \leftarrow \frac{1}{K} \sum_{n \in \mathcal{N}^{h}} G^{2}$; \label{alg:ps_estimate_aggregation_end}
        \
        % \State Aggregate the neural basis: $\mathbf{v}^{h + 1} \leftarrow \frac{1}{K} \sum_{n \in \mathcal{N}^{h}} \bar{\mathbf{v}}_{n}^{h}$;
        % \State Aggregate the coefficient (block-wise) and obtain $\mathbf{u}^{h + 1}$;
        \State Aggregate basis and coefficient to $\mathbf{v}^{h+1}$ and $\mathbf{u}^{h+1}$;\label{alg:ps_global_aggregation_end}
        \State Set $h \leftarrow h + 1$ and $c_{i}^{h} \leftarrow c_{i}^{h-1}$ ($\forall i \in [P^{2}]$);
		\EndWhile 
        \State Set $H \leftarrow h-1$ ,then send $\mathbf{v}^{H}$ and $\mathbf{u}^{H}$ to all clients.
	\end{algorithmic}
\end{algorithm}

\subsection{Preliminaries for Algorithm Design}
To solve the optimization problem in Eq. \eqref{eq:problem_formulation}, we first approximate the convergence bound. 
Specifically, we adopt an upper bound $\beta^{2}$ for the coefficient reducing error, where $\alpha_{n}^{h} \leq \beta^{2}$. 
Besides, the minimum loss value is approximated as zero, \ie, $F(\mathbf{x}^{*}) = 0$. 
Accordingly, the convergence bound in Eq. \eqref{eq:theorem_1} is formulated as follows:
\begin{equation}
    G(H, \tau) = \frac{4}{H \eta \tau} F(\mathbf{x}^{0}) + \frac{L \eta \tau }{3} ( G^{2} + 18 \sigma^{2}) + 6 L^{2} \beta^{2}
\end{equation}
% To ensure the convergence, we let this bound be less than $\gamma$, which is a positive number close to zero. 
% Generally, $G(H, \tau) \leq \gamma$ is equivalent to ensuring the contraint $F(\mathbf{x}^{H}) \leq \epsilon $ in Eq. \eqref{eq:problem_formulation}.

% It can be derived that the above convergence bound $G(H, \tau)$ will decrease as local updating frequency $\tau$ increases when $\tau \leq \sqrt{\frac{12 F(\mathbf{x}^{0})}{\eta^{2} H L (G^{2} + 18 \sigma^{2})}} $.
Since $\tau$ is a positive variable, the convergence bound $G(H, \tau)$ is a convex function with respect to the local update frequency $\tau$.
It can be derived that $G(H, \tau)$ will decrease as $\tau$ increases when $\tau \leq \small{\sqrt{\frac{12 F(\mathbf{x}^{0})}{\eta^{2} H L (G^{2} + 18 \sigma^{2})}}} $.
On the contrary, the trend of $G(H, \tau)$ and $\tau$ is the opposite.

To balance the completion time of heterogeneous clients, we first select the fastest client $l$ in round $h$ and let the completion time of other clients be approximately equal to that of client $l$, which can be formulated as follows:
\begin{equation} \label{eq:approximate_waiting_time}
    % \lfloor \frac{\tau_{n}^{h} \cdot \mu_{n}^{h} + \nu_{n}^{h}}{\tau_{l}^{h} \cdot \mu_{l}^{h} + \nu_{l}^{h}} \rfloor = 1, \qquad \forall n \in \mathcal{N}^{h}, \forall h
    0 \leq T_{l}^{h} - (\tau_{n}^{h} \cdot \mu_{n}^{h} + \nu_{n}^{h}) \leq \rho , \quad \forall n \in \mathcal{N}^{h}, \forall h
\end{equation} 

Notably, the completion time $T_{l}^{h}$ of client $l$ is the largest among that of all participating clients in round $h$.
Therefore, the total completion time can be denoted as follows:
\begin{equation}
    T(H, \tau) = \sum_{h=1}^{H} T_{l}^{h} = \sum_{h=1}^{H}(\tau_{l}^{h} \cdot \mu_{l}^{h} + \nu_{l}^{h}) 
\end{equation}

In order to minimize the convergence bound, 
we set the local update frequency $\tau_{l}^{h}$ of the fastest client $l$ in round $h$ as $\small{\sqrt{\frac{12 F(\mathbf{x}^{h})}{\eta^{2} H L (G^{2} + 18 \sigma^{2})}}}$. Thus, the optimization problem in Eq. \eqref{eq:problem_formulation} can be approximated as a univariate problem of finding the number of rounds $H$.

\centerline{$\mathop{\min} \sum_{h=1}^{H}(\tau_{l}^{h} \cdot \mu_{l}^{h} + \nu_{l}^{h})$ }
\begin{equation} \label{eq:approximate_problem_formulation}
    s.t.
    \begin{cases} 
    \tau_{l}^{h} = \sqrt{\frac{12 F(\mathbf{x}^{h})}{\eta^{2} H L (G^{2} + 18 \sigma^{2})}}, & \forall h  \\
    0 \leq T_{l}^{h} - (\tau_{n}^{h} \cdot \mu_{n}^{h} + \nu_{n}^{h}) \leq \rho , & \forall n \in \mathcal{N}^{h}, \forall h \\
    \mathcal{V}^{h} \leq \delta, & \forall h
    \end{cases} 
\end{equation}

% The first set of equations ensures a tight convergence bound.
% The second set of inequalities represents the requirement for average waiting time.
% The third set of inequalities  

\begin{algorithm}[t]
	\caption{Procedure at client $n$ in round $h$}\label{alg:client}
    \algnotext{EndFor}
    \algnotext{EndWhile}
    \algorithmicrequire{ global neural basis $\mathbf{v}^{h}$, reduced coefficient $\hat{\mathbf{u}}_{n}^{h}$, local update frequency $\tau^{h}_{n}$.} \\
	\algorithmicensure{ estimated variables $L_{n}$, $\sigma_{n}^{2}$ and $G_{n}^{2}$, updated neural basis $\bar{\mathbf{v}}^{h}_{n}$ and coefficient $\bar{\mathbf{u}}_{n}^{h}$}.
	\begin{algorithmic}[1]
        \State Receive $\mathbf{v}^{h}$, $\hat{\mathbf{u}}_{n}^{h}$ and $\tau^{h}_{n}$ from PS;
        \State Compose basis and coefficient $\hat{\mathbf{x}}^{h}_{n} \leftarrow \mathbf{v}^{h} \cdot \hat{\mathbf{u}}^{h}_{n}$;
        \State Initialize learning rate $\eta$ and set $\hat{\mathbf{x}}^{h}_{n}(0) \leftarrow \hat{\mathbf{x}}^{h}_{n}$;
        % \State 
        % \State Initialize the learning rate $\eta$;
		\For{each local iteration $t \in \{1, 2,...,\tau_{n}^{h}\}$}
		\State Update $\hat{\mathbf{x}}_{n}^{h} (t) \leftarrow \hat{\mathbf{x}}_{n}^{h} (t-1)-\eta \nabla F_{n} (\hat{\mathbf{x}}_{n}^{h} (t-1); \xi_{n}^{h})$;
		\EndFor
        \State Set $\bar{\mathbf{x}}_{n}^{h} \leftarrow \hat{\mathbf{x}}_{n}^{h} (\tau^{h}_{n})$;
		% \State {Estimate $L_{i} \leftarrow \frac{\|\nabla F_{i}(\bar{\mathbf{x}}_{n}^{h}) - \nabla F_{i}(\hat{\mathbf{x}}_{n}^{h})\|}{\|\bar{\mathbf{x}}_{n}^{h} - \hat{\mathbf{x}}_{n}^{h}\|}$};
        \State Estimate $L_{n} \leftarrow \|\nabla F_{n}(\bar{\mathbf{x}}_{n}^{h}) - \nabla F_{n}(\hat{\mathbf{x}}_{n}^{h}) \| / \|\bar{\mathbf{x}}_{n}^{h} - \hat{\mathbf{x}}_{n}^{h} \|$; \label{alg:client_estimate_begin}
		\State Estimate $\sigma_{n}^{2} \leftarrow\mathbb{E} [\|\nabla F_{n}(\hat{\mathbf{x}}_{n}^{h}, \xi^{n})-\nabla F_{n}(\hat{\mathbf{x}}_{n}^{h})\|^{2} ]$;
        \State Estimate $G_{n}^{2} \leftarrow\mathbb{E} [\|\nabla F_{n}(\hat{\mathbf{x}}_{n}^{h}, \xi^{n}) \|^{2} ]$; \label{alg:client_estimate_end}
		\State Decompose the updated local model $\bar{\mathbf{x}}^{h}_{n} \rightarrow \bar{\mathbf{v}}^{h} \cdot \bar{\mathbf{u}}^{h}_{n}$;
		\State Send $L_{n}$, $\sigma_{n}^{2}$, $G_{n}^{2}$, $\bar{\mathbf{v}}^{h}_{n}$ and $\bar{\mathbf{u}}_{n}^{h}$ to the PS.
	\end{algorithmic}
\end{algorithm}

\subsection{Algorithm Description} \label{subsec:algorithm_description}
In terms of Eq. \eqref{eq:approximate_problem_formulation}, we design a greedy-based control algorithm to adaptively assign proper coefficients and local update frequencies for heterogeneous clients. 
% In order to reduce the idle time and let every coefficient block be fully trained, we propose an efficient algorithm that dynamically adjusts the local update frequencies for heterogeneous clients .
% The proposed algorithms are formally described in Alg. \ref{alg:ps} and Alg. \ref{alg:client}, which state the procedure of PS and client, respectively.
The proposed algorithm consists of both the PS and client sides, which are formally described in Alg. \ref{alg:ps} and Alg. \ref{alg:client}, respectively.
We will introduce the algorithm in detail by the order of workflow in a training round.

Firstly, at the beginning of each round $h$, the algorithm determines the model width $p_{n}^{h}$ for each client $n \in \mathcal{N}^{h}$ (Lines \ref{alg:ps_determine_block_number_begin}-\ref{alg:ps_determine_block_number_end} of Alg. \ref{alg:ps}).
To minimize the reducing error, the algorithm greedily adds the coefficient blocks for each client as many as possible within a given maximum iteration time $\mu^{max}$ or the model width $p_{n}^{h}$ reaches the maximum value $P$.

Secondly, the algorithm selects the fastest client with the least completion time (Lines \ref{alg:ps_select_l_begin}-\ref{alg:ps_select_l_end} of Alg. \ref{alg:ps}).
Specifically, for each participating client $n \in \mathcal{N}^{h}$, the algorithm assumes it is the fastest client and solves the approximated problem in Eq. \eqref{eq:approximate_problem_formulation}, where the optimization object is $T_{n}(H, \tau_{n}) = \sum_{h'=h}^{H} (\tau_{n} \cdot \mu_{n}^{h'} + \nu_{n}^{h'})$ with $\tau_{n} = \sqrt{\frac{12 F(\mathbf{x}^{h})}{\eta^{2} H L (G^{2} + 18 \sigma^{2})}} $.
% Specifically, we set its local update frequency $\tau_{n} = \sqrt{\frac{12 F(\mathbf{x}^{h})}{\eta^{2} H L (G^{2} + 18 \sigma^{2})}} $ and taking it into $T_{n}(H, \tau_{n}) = \sum_{h'=h}^{H} (\tau_{n} \cdot \mu_{n}^{h'} + \nu_{n}^{h'})$.
% Then, we derived the number of rounds $H$ by minimizing $T_{n}$, and calculate corresponding $T_{n}$ and $\tau_{n}$ based on $H$.
Then, the number of rounds $H$ is obtained.
Accordingly, the total completion time for the entire training process $T_{n}$ is calculated according to $H$.
Then, the algorithm selects the fastest client $l$, \ie, $l \leftarrow \mathop{\arg\min}_{n \in \mathcal{N}^{h}} T_{n}$.
However, solving this problem requires information of the entire training process, such as clients' status and network bandwidth.
% Unfortunately, it is impossible to obtain these information in advance because these information are usually time-varing in the dynamic edge system.
Unfortunately, since these information are usually time-varying in the dynamic edge system, it is impossible to obtain them in advance.
To this end, we adopt the information in the current round to approximate the unavailable future information.
Therefore, the optimization object is approximated as follows:
\begin{equation} \label{eq:approximated_client_n_completion_time}
    T_{n}(H) = H \cdot ( \sqrt{\frac{12 F(\mathbf{x}^{h})}{\eta^{2} H L (G^{2} + 18 \sigma^{2})}} \cdot \mu_{n}^{h} + \nu_{n}^{h} )
\end{equation}
Notably, there are some variables, such as $L$, $\sigma^{2}$ and $G^{2}$, whose values are unknown at the beginning.
In order to address this issue, when $h = 0$, we adopt an identical predefined local update frequency $\mu_{1}$ for all participating clients, without performing the algorithm.
% When $h \geq 1$, we estimate these variables over clients' local loss functions (Lines \ref{alg:client_estimate_begin}-\ref{alg:client_estimate_end} of Alg. \ref{alg:client}) and aggregate them in PS (Line \ref{alg:ps_global_aggregation_begin} of Alg. \ref{alg:ps}) to obtain their specific values.
When $h \geq 1$, each participating client estimates these variables over its local loss function (Lines \ref{alg:client_estimate_begin}-\ref{alg:client_estimate_end} of Alg. \ref{alg:client}) and the PS aggregates them to obtain their specific values (Line \ref{alg:ps_global_aggregation_begin} of Alg. \ref{alg:ps}).


Thirdly, the algorithm determines other clients' local update frequencies based on the fastest client $l$'s completion time in round $h$, \ie, $T_{l}^{h}$ (Lines \ref{alg:ps_determine_other_tau_begin}-\ref{alg:ps_determine_other_tau_end} of Alg. \ref{alg:ps}).
Specifically, for each client $n \in \mathcal{N}^{h}$, the algorithm first derives a frequency space $[\tau_{a}, \tau_{b}]$ according to Eq. \eqref{eq:approximate_waiting_time} and searches the final local update frequency within this space, ensuring the waiting time does not exceed the threshold $\rho$.
Then, $(p_{n}^{h})^{2}$ blocks with the least total update times are selected to form the reduced coefficient $\hat{\mathbf{u}}_{n}^{h}$ for client $n$.
Finally, the algorithm searches the local update frequency $\tau_{n}^{h}$ in $[\tau_{a}, \tau_{b}]$ to minimize the variance among the total update times of all coefficient blocks.

Fourthly, the PS sends the global basis $\mathbf{v}^{h}$, reduced coefficient $\hat{\mathbf{u}}_{n}^{h}$ and local update frequency $\tau_{n}^{h}$ to each participating client $n$ for local training (\ie, Alg. \ref{alg:client}).
Once receiving the updated basis $\bar{\mathbf{v}}_{n}^{h}$ and coefficient $\bar{\mathbf{u}}_{n}^{h}$, as well as the estimated variables' values $L_{n}$, $\sigma^{2}_{n}$ and $G^{2}_{n}$, the PS performs global aggregation (Lines \ref{alg:ps_global_aggregation_begin}-\ref{alg:ps_global_aggregation_end} in Alg. \ref{alg:ps}).
The whole process continues until the total time cost exceeds the budget $T^{max}$.


==> fig/content/analysis.tex <==
In this section, we provide the convergence analysis of the proposed framework.
We first state the following assumptions, which are standard in non-convex optimization problems and widely used in the analysis of previous works \cite{jiang2023computation}.

\noindent\textbf{Assumption 1.} \textbf{(\textit{Smoothness})} The local objective function $F_{n}$ of each client $n$ is smooth with modulus $L$:
\begin{equation}
    \! \!F_{n}(\mathbf{y})\! - \!F_{n}(\mathbf{x}) \leq \frac{L}{2} \| \mathbf{y} - \mathbf{x} \|^{2} + \langle \nabla F_n(\mathbf{y}), \mathbf{y} - \mathbf{x} \rangle \quad \forall n, \mathbf{x}, \mathbf{y} 
\end{equation}

\noindent\textbf{Assumption 2.} \textbf{(\textit{Bounded Variance})} 
Let $\xi_{n}$ denote a random data batch sampled from client $n$'s local dataset $D_{n}$. 
% Let $D_{n}$ denote the local dataset of client $n$ and $\xi_{n}$ is a data batch randomly sampled from $D_{n}$.
There exists a constant $\sigma > 0$ such that the variance of stochastic gradients at each client is bounded by:
\begin{equation}
    \mathbb{E} [ \| \nabla F_{n}(\mathbf{x}; \xi_{n}) - \nabla F_{n} (\mathbf{x}) \|^{2} ] \leq \sigma^{2} \quad \forall \mathbf{x}, n, \xi_{n} 
\end{equation}
\vspace{0.1mm}
\noindent\textbf{Assumption 3.} \textbf{(\textit{Bounded Gradients})} There exists a constant $G>0$, such that the stochastic gradients at each client $n$ are bounded by:
\begin{equation}
    \mathbb{E} [ \| \nabla F_{n}(\mathbf{x}; \xi_{n}) \|^{2} ] \leq G^{2} \quad \forall \mathbf{x}, n, \xi_{n}  
\end{equation}
% For the convenience of analysis, we assume that all clients participate in training at each round (\ie, $K=N$). 
% For the convenience of analysis, we use the element-wise product to represent coefficients at different width.

% For the convenience of analysis, we represent the reduced coefficient by a block-wise product, \ie, $\hat{\mathbf{u}}^{h}_{n} = \mathbf{u}^{h} \odot \mathbf{m}^{h}_{n}$, where $\mathbf{u}^{h}$ is the global coefficient in round $h$ and $\mathbf{m}^{h}_{n}$ is the corresponding binary mask for client $n$ in round $h$. 
% Physically, the masked blocks are removed from the coefficient and the remaining blocks are composed with basis into the local model $\hat{\mathbf{x}}^{h}_{n}$, \ie, $\hat{\mathbf{x}}^{h}_{n} = \mathbf{v}^{h} \cdot (\mathbf{u}^{h} \odot \mathbf{m}^{h}_{n})$. 
% % To express the error induced by pruning coefficient, we adopt an upper bound $\beta^{2}$, where $\| \mathbf{u}^{h} - \hat{\mathbf{u}}^{h}_{n} \|^{2} \leq \beta^{2}$.
% After the neural composition, each client $n$ sets $\hat{\mathbf{x}}^{h}_{n} (0) = \hat{\mathbf{x}}^{h}_{n}$ and performs $\tau^{h}_{n}$ local iterations by mini-batch SGD optimizer over its local dataset $D_{n}$.
% Specifically, at each local iteration $t \in \{1, 2, \cdots, \tau^{h}_{n} \}$, the local model can updated as follows:
% \begin{equation}
%     \hat{\mathbf{x}}^{h}_{n}(t) = \hat{\mathbf{x}}^{h}_{n}(t-1) - \eta \nabla F_{n}(\hat{\mathbf{x}}^{h}_{n}(t-1); \xi_{n}) \odot \mathbf{m}_{n}^{h}
% \end{equation}
% where $\eta$ is the learning rate. 
In order to analyze the convergence bound of the global loss function after $H$ rounds, we present the following three important lemmas.

\noindent\textbf{Lemma 1.} According to Assumption 3, the deviations between global model $\mathbf{x}^{h}$ and local model $\hat{\mathbf{x}}^{h}_{n}(t-1)$ is bounded as:
\begin{align}
    & \! \! \! \! \sum_{t=1}^{\tau} \sum_{n=1}^{N} \mathbb{E} [\| \mathbf{x}^{h}\! -\! \hat{\mathbf{x}}_{n}^{h}(t\! -\! 1) \|^{2} ] \!\leq\! \frac{2 \tau^{3} \eta^{2} G^{2} N }{3} \! + \! 2 \tau \sum_{n=1}^{N} \alpha_{n}^{h} 
\end{align}
where $\alpha_{n}^{h}$ represents the model error induced by reducing coefficient for client $n$ in round $h$ (\ie, $ \alpha_{n}^{h} \triangleq  \|\mathbf{u}^{h} - \hat{\mathbf{u}}^{h}_{n} \|^{2}$) and $\tau = \mathop{\max_{n, h}} \{ \tau_{n}^{h} \}$.
 
\noindent\textbf{Lemma 2.} Combining Assumptions 1-2 and Lemma 1, the difference between global models in two successive rounds can be bounded as:
\begin{align}
    &  \mathbb{E} [\| \mathbf{x}^{h+1} - \mathbf{x}^{h} \|^{2}] \leq  3 \eta^{2} \tau^{2} \mathbb{E} [\|  \nabla F_{n} (\mathbf{x}^{h})  \|^{2}]  \notag \\
    & +  \frac{6 \eta^{2} \tau^{2} L^{2}}{N} \sum_{n=1}^{N} \alpha_{n}^{h} + 2 \tau^{4} \eta^{4} G^{2} L^{2} + 3 \eta^{2} \tau^{2} \sigma^{2} \label{eq:lemma_2}
\end{align}

\noindent\textbf{Lemma 3.} Under Assumption 1 and Lemma 1, the proposed framework ensures that:
\begin{align}
    &\mathbb{E}[\langle \nabla F(\mathbf{x}^{h}), \mathbf{x}^{h+1} - \mathbf{x}^{h} \rangle ]  \notag \\
    \leq & - \frac{\tau \eta}{2} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] + \frac{L^{2} \tau \eta}{N} \sum_{n=1}^{N} \alpha_{n}^{h} + \frac{\tau^{3} \eta^{3} L^{2} G^{2}}{3} \label{eq:lemma_3}
\end{align}

Let these assumptions and lemmas hold, then the convergence bound can be obtained as follows.

\noindent\textbf{Theorem 1.} If the learning rate satisfies $\eta \leq \frac{1}{6L\tau}$, the mean square gradient after $H$ rounds can be bounded as follows:

\begin{align}
    & \frac{1}{H} \sum_{h=0}^{H-1} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] \leq \frac{4}{H \eta \tau} (F(\mathbf{x}^{0}) - F(\mathbf{x}^{*})) \notag \\
    &  + \frac{6 L^{2}}{H N} \sum_{h=0}^{H-1} \sum_{n=1}^{N} \alpha_{n}^{h} + \frac{L \eta \tau }{3} ( G^{2} + 18 \sigma^{2} ) \label{eq:theorem_1}
\end{align}
where $\mathbf{x}^{*}$ denotes the optimal global model. 

\noindent\textit{Proof. } With the smoothness assumption, we have:
\begin{align}
    & \mathbb{E}[F(\mathbf{x}^{h+1})] - \mathbb{E}[F(\mathbf{x}^{h})] \notag \\
    \leq & \frac{L}{2} \mathbb{E} [\| \mathbf{x}^{h+1} - \mathbf{x}^{h} \|^{2}] + \mathbb{E}[\langle \nabla F(\mathbf{x}^{h}), \mathbf{x}^{h+1} - \mathbf{x}^{h} \rangle ] \label{eq:theorem_1_smooth} \\ 
    \leq & \frac{\tau \eta}{2}(3 \tau \eta L - 1) \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] + \frac{L^{2}\tau\eta}{N}(3 L \tau \eta + 1) \sum_{n=1}^{N} \alpha_{n}^{h} \notag \\
    & + \tau^{4} \eta^{4} L^{3} G^{2} + \frac{3 \eta^{2} \tau^{2} \sigma^{2} L}{2} + \frac{\tau^{3} \eta^{3} L^{2} G^{2}}{3} \label{eq:theorem_1_taking_lemmas_2_3}
\end{align}
where Eq. \eqref{eq:theorem_1_taking_lemmas_2_3} is obtained by inserting Eq. \eqref{eq:lemma_2} and Eq. \eqref{eq:lemma_3} into Eq. \eqref{eq:theorem_1_smooth}. Summing over the round $h \in \{0, 1, \cdots, H-1 \}$ on the both sides of Eq. \eqref{eq:theorem_1_taking_lemmas_2_3}, we have:
\begin{flalign}
    & \mathbb{E}[F(\mathbf{x}^{H})] - \mathbb{E}[F(\mathbf{x}^{0})] \leq \tau^{4} \eta^{4} L^{3} G^{2} H  \notag \\
    & + \frac{\tau \eta}{2}(3 \tau \eta L - 1) \sum_{h=0}^{H-1} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] + \frac{3 \eta^{2} \tau^{2} \sigma^{2} H L}{2} \notag \\
    & + \frac{L^{2}\tau\eta}{N}(3 L \tau \eta + 1) \sum_{h=0}^{H-1} \sum_{n=1}^{N} \alpha_{n}^{h} + \frac{\tau^{3} \eta^{3} L^{2} G^{2} H}{3} \label{eq:theorem_1_sum}
\end{flalign}
When the learning rate satisfies $\eta \leq \frac{1}{6L\tau}$, we can shift the terms in Eq. \eqref{eq:theorem_1_sum} as follows:
\begin{align}
    & \frac{\tau \eta}{4} \sum_{k=0}^{H-1} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] \leq \mathbb{E}[F(\mathbf{x}^{0})] - \mathbb{E}[F(\mathbf{x}^{H})] \notag \\
    & + \frac{3 L^{2} \tau \eta}{2 N} \sum_{h=0}^{H-1} \sum_{n=1}^{N} \alpha_{n}^{h} + \frac{\tau^{2} \eta^{2} H L}{12} ( G^{2} + 18 \sigma^{2} ) \label{eq:theorem_1_shift}
\end{align}

Finally, we divide both sides of Eq. \eqref{eq:theorem_1_shift} by $\frac{H \eta \tau}{4}$ to derive the convergence bound in Eq. \eqref{eq:theorem_1} of Theorem 1.

Thus, we complete the convergence analysis of the proposed framework under the non-convex setting.
The convergence bound is proportional to the coefficient reducing error. 
The larger the coefficient, the smaller the reducing error, leading to a tighter convergence bound.
Besides, the bound also depends on the local update frequency $\tau$, indicating that we can obtain better convergence performance by determining the local update frequency $\tau$ properly.








 

==> fig/content/conclusion.tex <==
In this paper, we have proposed a lightweight FL framework, called Heroes, to address the challenges of resource limitation and client heterogeneity with the enhanced neural composition and adaptive local update.
We have analyzed the convergence of Heroes and designed a greedy-based algorithm to jointly assign proper tensors and local update frequency for each client, which enables every parameter in the global model to benefit from all clients' knowledge and get fully trained.
Extensive experiments demonstrate the effectiveness and advantages of our proposed framework.

==> fig/content/evaluation.tex <==
\subsection{Datasets and Models}

\subsubsection{\textbf{Datasets}}
We conduct the experiments over three common datasets: CIFAR-10\cite{krizhevsky2009learning}, ImageNet\cite{russakovsky2015imagenet} and Shakespeare\cite{caldas2018leaf}.
Specifically, CIFAR-10 is an image dataset including 60,000 images (50,000 images for training and 10,000 images for testing), which are 3$\times$32$\times$32 dimensional and evenly from 10 classes.
ImageNet contains 1,281,167 training images, 50,000 validation images and 100,000 test images from 1,000 classes and is more challenging to train the models for visual recognition.
Considering the constrained resource of edge clients, we create a subset of ImageNet, called ImageNet-100, that consists of 100 out of 1,000 classes.
Besides, each image's resolution is resized to 3$\times$144$\times$144.
Shakespeare is a text dataset for next-character prediction built from Shakespeare Dialogues, and includes 422,615 samples with a sequence length of 80.
We split the dataset into 90\% for training and 10\% for testing \cite{caldas2018leaf}.
CIFAR-10 and ImageNet-100 represent the low-resolution and high-resolution computer vision (CV) learning tasks, respectively, while Shakespeare represents the natural language processing (NLP) learning task.

% In order to simulate the data heterogeneity, we adopt two different data partition schemes for the two image datasets, respectively, \ie, latent Dirichlet allocation (LDA) and skewed label, which are well explored in previous works \cite{wang2022accelerating}.
% \textbf{(1) LDA for CIFAR-10:} $\varGamma$ ($\varGamma =$ 0.2, 0.4, 0.6 and 0.8) of the samples on each client belong to one calss and the remaining samples evenly belong to other classes, where $\varGamma = $ 1 represents IID.
% \textbf{(2) Skewed label for ImageNet-100:} Each client lacks $\varGamma$ ($\varGamma =$ 20, 40, 60 and 80) classes of samples and the data volume of each class is balanced, where $\varGamma = $ 0 represents IID.
% Since the Shakespeare dataset is a natural Non-IID dataset where each speaking role in each play is considered as a different client, 
% For the text dataset Shakespeare, we follow \cite{caldas2018leaf} to natuarlly consider each speaking role in each paly as a different client.
\subsubsection{\textbf{Data Distribution}}
To simulate the non-independent and identically distributed (Non-IID) data, we adopt three different data partition schemes for the three datasets, respectively.
Specifically, we adopt latent Dirichlet allocation (LDA) over CIFAR-10 \cite{jiang2023heterogeneity}, where $\varGamma$\% ($\varGamma =$ 20, 40, 60 and 80) of the samples on each client belong to one class and the remaining samples evenly belong to other classes. 
Particularly, $\varGamma =$ 10 represents the IID setting.
For ImageNet-100, we control that each client lacks $\phi$ ($\phi =$ 20, 40, 60 and 80) classes of samples and the data volume of each class is the same \cite{wang2022accelerating}, where $\phi = $ 0 represents the IID setting.
In our experiments, both $\varGamma$ and $\phi$ are set to 40 by default.
Shakespeare is a natural Non-IID dataset, where the dialogues of each speaking role in each play are regarded as the local data of a specific client \cite{caldas2018leaf} and the Non-IID level is fixed.
For fair comparison, the full test datasets are used to evaluate the models' performance.

\subsubsection{\textbf{Models}}
To validate the universality of the enhanced neural composition technique, we conduct the experiments across several different architectures. 
Firstly, a 4-layer CNN with three 3$\times$3 convolutional layers and one linear output layer is adopted for the CIFAR-10 dataset.
% where the hidden size of each layer is 64, 128 and 128, respectively.
Secondly, we utilize the standard ResNet-18 for the more challenging ImageNet-100 dataset.
Thirdly, for the Shakespeare dataset, we adopt an RNN model and set both the hidden channel size and embedding size to 512 \cite{mei2022resource}.

% \vspace{-2mm}
\subsection{Baselines and Metrics}
\subsubsection{\textbf{Baselines}}
We choose the following four baselines for performance comparison:
\ding{172} \textit{FedAvg} \cite{mcmahan2017communication} transmits and trains the entire models with a fixed (non-dynamic) and identical (non-diverse) local update frequency for all clients.
\ding{173} \textit{ADP} \cite{wang2018edge} dynamically determines the identical local update frequency for all clients in each round on the basis of the constrained resource.
\ding{174} \textit{HeteroFL} \cite{diao2020heterofl} reduces the model width for each client based on its computation power by model pruning.
\ding{175} \textit{Flanc} \cite{mei2022resource} utilizes the neural composition technique to adjust the model width, where the coefficients in different shapes do not share any parameter.

\subsubsection{\textbf{Metrics}}
We employ the following four metrics to evaluate the performance of Heroes and baselines.
\ding{172} \textit{Test accuracy} is measured by the proportion between the amount of the correct samples through model inference and that of all test samples. 
\ding{173} \textit{Average Waiting Time} is calculated by averaging the time each client waits for global aggregation in a round, reflecting the impact of client heterogeneity.
\ding{174} \textit{Completion time} is defined as the total time cost to reach the target accuracy, which reflects the training speed.
\ding{175} \textit{Network Traffic} is the overall size of models (or tensors) transmitted between PS and clients during the training process, which quantifies the communication cost.

% \subsubsection{\textbf{Simulation Platform}}
\subsection{Experimental Setup}
The experimental environment is built on an AMAX deep learning workstation equipped with an Intel Xeon 5218 CPU, 8 NVIDIA GeForce RTX 3090 GPUs and 256GB RAM.
We simulate an FL system with 100 virtual clients and one PS (each is implemented as a process in the system) on this workstation.
In each round, we randomly activate 10 clients to participate in training.
Specifically, the model training and testing are implemented based on the PyTorch framework\footnote{https://pytorch.org/docs/stable}, and the MPI for Python library\footnote{https://mpi4py.readthedocs.io/en/stable/} is utilized to build up the communication between clients and the PS.

To reflect heterogeneous and dynamic network conditions, we let each client's download speed to fluctuate between 10Mb/s and 20Mb/s \cite{wang2022accelerating}. 
Since the upload speed is usually smaller than the download speed in typical WANs, we configure it to fluctuate between 1Mb/s and 5Mb/s \cite{jiang2023heterogeneity} for each client. 
Besides, considering the clients' computation capabilities are also heterogeneous and dynamic, the time cost of one local iteration on a certain simulated client follows a Gaussian distribution whose mean and variance are derived from the time records on a physical device (\eg, laptop, TX2, Xavier NX, AGX Xavier) \cite{liao2023adaptive}.


\subsection{Evaluation Results}
\subsubsection{\textbf{Training Performance}}
We implement Heroes and baselines on CIFAR-10 and ImageNet-100 to observe their training performance (\eg, test accuracy).
% The test accuracy with respect to completion time of five schemes is shown in Fig. \ref{fig:image_dataset_acc_time}.
The results in Fig. \ref{fig:image_dataset_acc_time} show that Heroes converges much faster than the baselines while accomplishing a comparable accuracy.
For instance, by Fig. \ref{fig:cifar_acc_time}, Heroes takes 1,375s to achieve an accuracy of 70\% for CNN on CIFAR-10, while FedAvg, ADP, HeteroFL and Flanc take 4,508s, 3,924s, 3,015s and 3,187s, respectively.
In other words, Heroes can speed up the training process by up to 2.67$\times$ compared to the baselines.
Besides, the model's accuracy in Heroes also surpasses that in the baselines within a given completion time.
For example, Heroes achieves an accuracy of 64.36\% after training ResNet-18 over ImageNet-100 for 40,000s, while that of FedAvg, ADP, HeteroFL and Flanc is 55.22\%, 56.34\%, 52.11\% and 51.89\%, respectively.
In general, within the same time budget, Heroes can improve the test accuracy by about 10.46\% compared with the baselines.
These results demonstrate the advantages of Heroes in accelerating model training.

\subsubsection{\textbf{Impact of Client Heterogeneity}}
To evaluate the impact of client heterogeneity on model training with different schemes, we illustrate the average waiting time each round among the participating clients in Fig. \ref{fig:image_dataset_waiting_time}.
The results show that Heroes incurs much less waiting time than the baselines, which means high robustness against system heterogeneity.
For example, by Fig. \ref{fig:waiting_time_cifar}, the average waiting time in Heroes is 2.86s when training CNN over CIFAR-10, while that in FedAvg, ADP, HeteroFL and Flanc is 15.37s, 11.02s, 8.34s and 5.96s, respectively.
Specifically, both FedAvg and ADP assign the entire model and identical local update frequencies for all clients during each round without considering the system heterogeneity, resulting in non-negligible waiting time.
HeteroFL and Flanc reduce the model width for different clients according to their various computation power.
However, they ignore the heterogeneity in clients' communication capabilities.
For example, the client with a slow upload speed will easily become the straggler and delay the global aggregation.
In addition to reducing the model width, Heroes also adjusts the local update frequencies for different clients to balance their completion time in each round.
Therefore, Heroes can diminish the impact or system heterogeneity significantly.

\begin{figure}[t]
	\centering
	\subfigure[CNN on CIFAR-10.]{
		\includegraphics[width=1.6in]{fig/cnn_acc_time_4.eps}\label{fig:cifar_acc_time}
	}
	\subfigure[ResNet-18 on ImageNet-100.]{
		\includegraphics[width=1.6in]{fig/image_acc_time_4.eps}\label{fig:image_acc_time}
	}
    \vspace{-2mm}
	\caption{Training performance of different schemes.}\label{fig:image_dataset_acc_time}
	\vspace{-3mm}
\end{figure}

\begin{figure}[t]
	\centering
	\subfigure[CNN on CIFAR-10.]{
		\includegraphics[width=1.6in]{fig/cnn_idle_time.eps}\label{fig:waiting_time_cifar}
	}
	\subfigure[ResNet-18 on ImageNet-100.]{
		\includegraphics[width=1.6in]{fig/image_idle_time.eps}\label{fig:waiting_time_image}
	}
    \vspace{-2mm}
	\caption{Average waiting time of different schemes.}\label{fig:image_dataset_waiting_time}
	\vspace{-3mm}
\end{figure}

\subsubsection{\textbf{Resource Consumption}}
We observe the resource consumption (\eg, network traffic and completion time) of five schemes when they achieve different target accuracies on the two image datasets (\eg, 75\% on CIFAR-10, 60\% on ImageNet-100).
The results in Fig. \ref{fig:cifar_resource} and Fig. \ref{fig:image_resource} demonstrate that Heroes can mitigate both the time and traffic costs greatly.
For instance, in Fig. \ref{fig:image_traffic}, to obtain the target accuracy of 50\% on ImageNet-100, the traffic cost of Heroes is 17.81GB, while that of FedAvg, ADP, HeteroFL and Flanc is 82.34GB, 77.75GB, 62.87GB and 49.38GB, respectively.
At the same time, by Fig. \ref{fig:image_time}, Heroes can separately speed up the training process by about 3.09$\times$, 2.86$\times$, 3.15$\times$ and 2.81$\times$, compared with FedAvg, ADP, HeteroFL and Flanc. 
In a word, Heroes achieves the target accuracy fastest with about 2.97$\times$ speedup while reducing the network traffic by about 72.05\% compared with the baselines.


\begin{figure}[t]
	\centering
	\subfigure[Traffic Overhead.]{
		\includegraphics[width=1.6in]{fig/cnn_traffic_4.eps}\label{fig:cifar_traffic}
	}
	\subfigure[Completion Time.]{
		\includegraphics[width=1.6in]{fig/cnn_time_4.eps}\label{fig:cifar_time}
	}
    \vspace{-2mm}
	\caption{The resources consumption of CNN on CIFAR10.}\label{fig:cifar_resource}
	\vspace{-3mm}
\end{figure}




\subsubsection{\textbf{Impact of Non-IID Data}}
We test these schemes' test accuracies over the CIFAR-10 and ImageNet-100 datasets under different Non-IID levels within a given completion time (800s for CIFAR-10 and 40,000s for ImageNet-100).
The results in Fig. \ref{fig:image_dataset_non_iid_level} indicate that the test accuracy decreases as the Non-IID level increases for all schemes.
For instance, by Fig. \ref{fig:non_iid_level_cifar}, when training CNN on CIFAR-10 with $\varGamma=80$, Heros achieves an accuracy of 68.9\%, which is 14.72\%, 13.21\%, 7.48\% and 24.08\% higher than FedAvg, ADP, HeteroFL and Flanc, respectively.
Heroes investigates the benefits of neural composition technique and adaptive control of local update frequency, which can accelerate the FL process while maintaining the accuracy of the complete model.
Compared to FedAvg and ADP, Heroes will perform more training rounds to achieve higher accuracy within the given time.
Compared to HeteroFL and Flanc, Heroes enables every parameter in the global model to be fully trained over the full range of knowledge, thus eliminating the training bias and achieving better performance.

% Heroes integrates the adaptive control of neural composition and local update frequency, so as to improve the training efficiency while allowing different parts of the global model to be evenly trained.
% Compared to FedAvg and ADP, which train the complete model, Heroes 



\begin{figure}[t]
	\centering
	\subfigure[CNN on CIFAR-10.]{
		\includegraphics[width=1.6in]{fig/cnn_non_iid.eps}\label{fig:non_iid_level_cifar}
	}
	\subfigure[ResNet-18 on ImageNet-100.]{
		\includegraphics[width=1.6in]{fig/image_non_iid.eps}\label{fig:non_iid_level_image}
	}
    \vspace{-2mm}
	\caption{Training performance under different Non-IID levels.}\label{fig:image_dataset_non_iid_level}
	\vspace{-3mm}
\end{figure}

\begin{figure}[t]
	\centering
	\subfigure[Traffic Overhead.]{
		\includegraphics[width=1.6in]{fig/image_traffic_4.eps}\label{fig:image_traffic}
	}
	\subfigure[Completion Time.]{
		\includegraphics[width=1.6in]{fig/image_time_4.eps}\label{fig:image_time}
	}
    \vspace{-2mm}
	\caption{The resource consumption of ResNet-18 on ImageNet-100.}\label{fig:image_resource}
	\vspace{-3mm}
\end{figure}

% \vspace{12mm}
\begin{figure}[t]
	\centering
	\subfigure[Test Accuracy vs.Time.]{
		\includegraphics[width=1.59in]{fig/rnn_acc_time.eps}\label{fig:rnn_acc_time}
	}
	\subfigure[Traffic Overhead.]{
		\includegraphics[width=1.59in]{fig/rnn_traffic.eps}\label{fig:rnn_traffic}
	}
    \vspace{-2mm}
	\caption{The performance of training RNN over Shakespeare}\label{fig:text_dataset_performance}
	\vspace{-3mm}
\end{figure}







\subsubsection{\textbf{Performance on Text Dataset}}
Finally, to verify the generalization of the enhanced neural composition technique, we conduct a set of experiments to train RNN over the text dataset Shakespeare.
The results in Fig. \ref{fig:text_dataset_performance} demonstrate that Heroes can also accomplish better training performance than the baselines on the NLP learning task.
Specifically, according to Fig. \ref{fig:rnn_acc_time}, Heroes takes 1,862s to reach the target accuracy of 45\%, while FedAvg, ADP, HeteroFL and Flanc take 4,183s, 4,015s, 3,182s and 2,874s, respectively.
% Specifically, by Fig.\ref{fig:rnn_acc_time}, the test accuracy of Heroes is 49.04\%, while that of FedAvg, ADP, HeterFL and Flanc is 46.27\%, 47.13\%, 45.43\% and 45.86\%, respectively, with the completion time 600s.
Besides, by Fig. \ref{fig:rnn_traffic}, compared with FedAvg, ADP, HeteroFL and Flanc, Heroes saves about 60.71\%, 42.57\%, 38.65\% and 26.72\% of network traffic, respectively.
Therefore, compared with baselines, Heroes can provide up to 1.91$\times$ speedup and reduce the traffic consumption by about 45.06\% when training RNN over Shakespeare.





% \begin{figure}[t]
% 	\centering
% 	\subfigure[Traffic Overhead.]{
% 		\includegraphics[width=1.6in]{fig/rnn_traffic.eps}\label{fig:rnn_traffic}
% 	}
% 	\subfigure[Completion Time.]{
% 		\includegraphics[width=1.6in]{fig/rnn_time.eps}\label{fig:rnn_time}
% 	}
% 	\caption{The resource consumption of RNN over Shakespeare.}\label{fig:rnn_resource}
% 	\vspace{-3mm}
% \end{figure}



==> fig/content/framework.tex <==
To enhance the training efficiency and resource utilization for FL, we propose a lightweight FL framework, called Heroes, which integrates the benefits of enhanced neural composition and adaptive local update.
Specifically, in Heroes, there are three main phases in each round as follows.

\subsubsection{\textbf{Tensors and Frequency Assignment}}
The PS first determines the model width $p_{n}^{h}$ for each client $n$ in round $h$.
As studied in \cite{diao2020heterofl, mei2022resource}, the smaller the model width, the less the required computation resource.
To alleviate the performance degradation, Heroes increases each client's model width as much as possible within its resource budget.
Then, for each client $n$, Heroes selects $(p_{n}^{h})^{2}$ coefficient blocks with the least total update times as the reduced coefficient $\hat{\mathbf{u}}_{n}^{h}$.
Finally, Heroes assigns a proper local update frequency $\tau_{n}^{h}$ to each client $n$ by the algorithm proposed in Section \ref{subsec:algorithm_description} to minimize the idle waiting time and balance the training across different coefficient blocks. 

\subsubsection{\textbf{Local Training}}
In round $h$, each client $n \in \mathcal{N}^{h}$ first downloads the latest neural basis $\mathbf{v}^{h}$ and the reduced coefficient $\hat{\mathbf{u}}_{n}^{h}$ from the PS, then composes them into the local model $\hat{\mathbf{x}}_{n}^{t}$.
Each local model $\hat{\mathbf{x}}_{n}^{t}$ is trained over the local dataset $D_{n}$ for $\tau_{n}^{h}$ iterations.
Let $\bar{\mathbf{x}}_{n}^{h}$ represent the updated local model of client $n$ in round $h$.
After the local training, $\bar{\mathbf{x}}_{n}^{h}$ is be decomposed into the updated neural basis $\bar{\mathbf{v}}_{n}^{h}$ and coefficient $\bar{\mathbf{u}}_{n}^{h}$, \ie, $\bar{\mathbf{x}}_{n}^{h} \approx \bar{\mathbf{v}}_{n}^{h} \cdot \bar{\mathbf{u}}_{n}^{h}$.
Since the size of low-rank tensors is inherently smaller than that of original model, each client $n$ uploads $\bar{\mathbf{v}}_{n}^{h}$ and $\bar{\mathbf{u}}_{n}^{h}$, instead of $\bar{\mathbf{x}}_{n}^{h}$, to the PS for global aggregation, which further saves the limited bandwidth.

\subsubsection{\textbf{Global Aggregation}}
In round $h$, upon receiving the updated neural basis and coefficient from all the participating clients in $\mathcal{N}^{h}$, the PS performs global aggregation to obtain the latest basis $\mathbf{v}^{h+1}$ and coefficient $\mathbf{u}^{h+1}$ for the next round of training.
For neural basis, Heroes directly averages the updated ones from all participating clients, \ie, $\mathbf{v}^{h+1} = \frac{1}{K} \sum_{n=1}^{K} \bar{\mathbf{v}}_{n}^{h}$.
For coefficient, Heroes performs the block-wise aggregation.
Specifically, let $i \in \{1, 2, \cdots, P^{2} \}$ represent the block index and $\mathcal{N}_{i}^{h}$ denote the set of clients that train the $i$-th coefficient block in round $h$. 
The latest $i$-th coefficient block $\mathbf{u}^{h+1, i}$ is obtained as follows:
\begin{equation}
    \mathbf{u}^{h+1, i} = \frac{1}{|\mathcal{N}_{i}^{h}|} \sum_{n \in \mathcal{N}_{i}^{h}} \bar{\mathbf{u}}_{n}^{h, i}
\end{equation}
where $\bar{\mathbf{u}}_{n}^{h, i}$ represents the $i$-th coefficient block updated by client $n$ in round $h$.
For instance, as shown in Fig. \ref{fig:framework}, the leftmost block is trained by two clients (\ie, 2 and 4), thus its value is $3 = \frac{1}{2} \times (4+2)$.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{fig/framework_v2.pdf}
    \caption{The demonstration of the proposed framework.} \label{fig:framework}\vspace{-5mm}
\end{figure}

For better explanation of Heroes, we give a demonstration of Heroes in Fig. \ref{fig:framework}. 
Four heterogeneous clients participate in training, which are divided into three levels by their computation power, \ie, \textit{weak} smartphones (clients 1 and 3), \textit{medium} laptop (client 2) and \textit{powerful} PC (client 4).
The complete coefficient contains three blocks.
Heroes selects one coefficient block for the \textit{weak} clients 1 and 3, and two blocks for \textit{medium} client 2.
The \textit{powerful} client 4 utilizes all three blocks for model training.
We adopt the block's color to denote the amount of training it has obtained.
Specifically, the total update times of blue blocks is ample, while that of orange blocks and white blocks is moderate and few, respectively.
To ensure sufficient training for every block, the selected blocks are the least trained ones currently.
Besides, Heroes assigns different local update frequencies for these four clients to balance their completion time.
For example, the \textit{weak} client 1 trains the model much slower than the \textit{powerful} client 4.
Thus, client 1 performs fewer local iterations (\eg, 10) to alleviate the straggler effect, while client 4 performs more local iterations (\eg, 30) to make more contributions to the global model.
In addition to the balance of clients' completion time, the balance of coefficient blocks' total update times is also considered for the determination of each client's local update frequency.

 
% Finally, the latest coefficient $\mathbf{u}^{h+1}$ is obtained by combining these aggregated blocks by order. 
% Heroes selects one coefficient block for clients 1 and 3, respectively, and selects two blocks for client 2.
% Additionally, the training evenness of different coefficient blocks is also considered for the determination of each client's local update frequency.
% Then, we adjust the local update frequencies for different clients by the algorithm proposed in Section \ref{subsec:algorithm_description} to minimize the system idle time as well as keep the training consistency among each coefficient blocks.
% Finally, the PS performs block-wise aggregation on local coefficients.
% The block 3 is trained by three clients (\ie, 2, 3 and 4), thus its value is $4 = \frac{1}{3} \times (3+6+3)$.
% Then, client $n$ composes basis and coefficient into the local model $\hat{\mathbf{x}}_{n}^{t}$, and trains $\hat{\mathbf{x}}_{n}^{t}$ over its local dataset $D_{n}$ for $\tau_{n}^{h}$ iterations. 
% After the local training, $\bar{\mathbf{x}}_{n}^{h}$ will be uploaded to the PS for global aggregation.
% $\bar{\mathbf{x}}_{n}^{h}$ is decomposed before the communication to save the limited bandwidth, \ie, $\bar{\mathbf{x}}_{n}^{h} \approx \bar{\mathbf{v}}_{n}^{h} \cdot \bar{\mathbf{u}}_{n}^{h}$. 
% Finally, client $n$ uploads updated neural basis $\bar{\mathbf{v}}_{n}^{h}$ and coefficient $\bar{\mathbf{u}}_{n}^{h}$ to the PS.


==> fig/content/intro.tex <==
In traditional machine learning approaches, data is gathered from various sources and transmitted to a central server for model training. 
However, in edge computing (EC), where data is generated and processed at the edge clients, this centralized approach becomes infeasible due to privacy concerns \cite{liu2022enhancing}.
Federated Learning (FL) \cite{mcmahan2017communication} is an emerging paradigm that enables collaborative model training across distributed clients, bringing the power of machine learning to EC \cite{gao2019auction}. 
As the field of FL continues to evolve, it carries significant potential to advance edge computing capabilities and facilitate intelligent applications across diverse domains, such as healthcare, smart cities and autonomous vehicles\cite{kairouz2021advances}.


However, it is difficult to implement efficient FL in practical edge networks due to resource limitation \cite{liu2023finch}, which primarily revolve around constrained computation resources and scarce communication resources on edge clients, such as smartphones and Internet of Things (IoT) devices.
Firstly, edge clients often have limited computation capabilities, especially compared to high-performance devices like desktop GPUs \cite{ignatov2019ai}.
For example, the floating-point operations per second (FLOPS) of an iPhone14 is only about 5\% of that of the desktop GPU RTX3090.
Secondly, the communication resources are also scarce in edge networks \cite{liu2023yoga}.
The bandwidth of wide area networks (WANs) between the PS and edge clients is much lower (\eg, 15$\times$) than that of local area networks (LANs) within the data centers \cite{wang2021resource}.
Unfortunately, the growing complexity (\eg, parameter size or architecture) of deep neural networks (DNNs) further intensifies the consumption of both computation and communication resources. 
For instance, a standard ResNet-18 \cite{he2016deep} consists of 11.68 million parameters and requires 27.29 billion floating-point operations (FLOPs) to process a single image, making the local update process extremely slow or even infeasible on edge clients \cite{jiang2022fedmp}.
Besides, the frequent transmissions of a large number of parameters will also strain the limited network bandwidth.

Some previous works have made efforts to address the challenge of resource limitation in FL by employing various techniques, such as gradient compression \cite{li2021talk, liu2022communication} and model pruning \cite{diao2020heterofl, horvath2021fjord}. Specifically, \textit{FlexCom} \cite{li2021talk} and \textit{AdaGQ} \cite{liu2022communication} compress the transmitted gradients by sparsification or quantization to alleviate the communication overhead.
However, these approaches do not reduce the model complexity and the computation overhead is still high.
To save both the computation and communication resources, \textit{HeteroFL} \cite{diao2020heterofl} and \textit{Fjord} \cite{horvath2021fjord} propose to prune the complete model into the smaller sub-models for training.
Nevertheless, excessive parameter pruning will significantly degrade training performance.
For instance, \textit{HeteroFL} prunes 93.75\% of the parameters from the complete model to accommodate the limitations (\eg, CPU power, RAM, energy) on weak clients like smartphones, leaving only 6.25\% of the parameters to be optimized. 
As a result, the majority of parameters are unable to benefit from the local data on these weak clients, leading to poor training performance of the complete model.


To address the above issues, \textit{Flanc} \cite{mei2022resource} proposes the neural composition technique, which approximates each model weight as the product of two low-rank tensors, named neural basis and coefficient.
Concretely, the models of various complexities are constructed by composing (\ie, multiplying) the neural basis with the coefficient of different sizes.
In each round, the parameter server (PS) sends the neural basis and a proper coefficient to each client for composition and local training.
The entire neural basis is trained by all clients and its learned knowledge can be propagated to all parameters, which enables every parameter to access the full range of knowledge.
We observe that the size of low-rank tensors is inherently much smaller than that of the original model.
For example, the size of standard ResNet-18 is 42.8MB, while that of approximated tensors is only 15.3MB.
Thus, this approach can reduce both computation and communication consumption during training.

Despite resource efficiency, the neural composition technique will encounter some problems in the context of FL.
Firstly, \textit{Flanc} only aggregates the coefficients with the same shape.
As a consequence, the coefficient of a specific shape is only trained by the clients with the corresponding computation power, which may be insufficient for global model convergence.
This issue becomes more prominent when high-performance clients only constitute a small fraction of all clients in the EC system due to their expensive price. For instance, the largest coefficient is only trained by a few powerful clients.
As a result, the largest global model may struggle to converge within the given completion time, leading to poor training performance.
Secondly, the edge clients are equipped with different hardware, thus their capabilities (\eg, CPU power, bandwidth) may vary significantly \cite{li2022pyramidfl}, \ie, client heterogeneity, which poses a great impact on training efficiency.
For example, if the PS sends the neural basis and a large coefficient to a client with strong computation power but low upload bandwidth, the completion time for model updates will be prolonged, causing long delays in the aggregation step. 

In order to tackle the aforementioned challenges, we propose a lightweight FL framework, called Heroes (Lig\textbf{H}tweight F\textbf{e}derated Lea\textbf{r}ning thr\textbf{o}ugh N\textbf{e}ural Compo\textbf{s}ition).
On the one hand, we enhance the neural composition technique to aggregate the coefficients with different shapes into the largest one.
Besides, by adaptively assigning the coefficients to clients, each parameter in the global coefficient can be fully trained, ensuring global model convergence.
On the other hand, we adjust the local update frequencies for different clients to balance their completion time, so as to diminish the impact of client heterogeneity and improve the training efficiency.
Nevertheless, the neural composition and local update frequency are interconnected. 
Specifically, the completion time depends on the size of composed model, which affects the determination of local update frequency.
Meanwhile, the local update frequency also affects the training adequacy of each parameter in coefficient.
Therefore, \textit{it is necessary yet challenging to jointly assign proper coefficient and local update frequency for each client.}
Our contributions are summarized as follows:
\begin{itemize}
    \item We propose a lightweight FL framework, called Heroes, which overcomes the challenges of resource limitation and client heterogeneity through enhanced neural composition and adaptive local update. Besides, a theoretical convergence analysis is provided for Heroes.
    \item  Guided by the convergence bound, we design a greedy-based algorithm to adaptively assign the proper coefficients and local update frequencies for participating clients based on both their heterogeneous capabilities and resource budgets.
    \item The performance of Heroes is evaluated through extensive experiments and the results demonstrate that Heroes can reduce the traffic consumption by about 72.05\% and provide up to 2.97$\times$ speedup for the training process compared to the baselines.
\end{itemize}






















==> fig/content/motivation.tex <==
\subsection{Federated Learning}
Considering a client set $\mathcal{N} = \{1, 2, \cdots, N \}$ coordinated by the PS, each client $n \in \mathcal{N}$ holds its local dataset $D_{n} = \{\zeta_{i}^{n}\}_{i=1}^{|D_{n}|}$, where $\zeta_{i}^{n}$ denotes a data sample from $D_{n}$.
Further, we represent the loss function as $\mathcal{L}(\mathbf{x}; \zeta)$, which measures how well the model $\mathbf{x}$ performs on data sample $\zeta$.
Therefore, the local loss function of client $n$ is defined as:
\begin{equation}
    F_{n}(\mathbf{x}) \triangleq \mathbb{E}_{\zeta \thicksim D_{n}} [\mathcal{L}(\mathbf{x}; \zeta)] 
\end{equation}

The global loss function is a linear combination of all $N$ clients, and the goal of FL is to train a high-quality model $\mathbf{x}^{*}$ with minimum global loss function, which is defined as:
\begin{equation} \label{eq:fl_goal}
    \mathbf{x}^{*} \triangleq  \mathop{\arg\min}_{\mathbf{x}} F(\mathbf{x}) = \mathop{\arg\min}_{\mathbf{x}} \frac{1}{N} \sum_{n=1}^{N} F_{n} (\mathbf{x})
\end{equation}


Suppose there are $H$ rounds of training in total. 
In each round $h \in \{1, 2, \cdots, H\}$, the PS randomly selects a set of clients $\mathcal{N}^{h} \subseteq  \mathcal{N}$ to participate in training and sends the fresh global model $\mathbf{x}^{h}$ to the specified clients, where $|\mathcal{N}^{h}| = K$.
Then, each client $n \in \mathcal{N}^{h}$ updates the global model $\mathbf{x}^{h}$ over its local dataset $D_{n}$ for $\tau$ times, where each update is regarded as one local iteration and $\tau$ represents the local update frequency.
Let $\mathbf{x}^{h}_{n} (t)$ denote the local model of client $n$ at iteration $t$ in round $h$.
For the mini-batch stochastic gradient descent (SGD) \cite{yu2019parallel} algorithm, a local iteration can be expressed as follows:
\begin{equation}
    \mathbf{x}^{h}_{n} (t+1) = \mathbf{x}^{h}_{n} (t) - \eta \nabla F_{n} (\mathbf{x}^{h}_{n} (t); \xi^{n})
\end{equation}
where $\xi^{n}$ denotes a random data batch from the local dataset $D_{n}$ and $\eta$ is the learning rate.
Finally, the PS collects the updated local models from the participating clients and aggregates them to the latest global model for further training, \ie, $ \mathbf{x}^{h+1} = \frac{1}{N} \sum_{n=1}^{N} \mathbf{x}^{h}_{n} (\tau)$.


\subsection{Enhanced Neural Composition}
To make full use of the limited resources, it is necessary to adjust the complexity of local model for each client based on its resource budgets \cite{diao2020heterofl, horvath2021fjord, mei2022resource}.
Herein, we follow \textit{Flanc} \cite{mei2022resource} to innovatively propose an enhanced neural composition technique to construct the models in different widths (\ie, the number of hidden channels in each weight) based on low-rank factorization \cite{phan2020stable}. Concretely, since the weights in DNNs are usually over-parameterized \cite{zou2019improved}, each layer's weight (\eg, convolution, fully connection) can be approximated as the product of two low-rank tensors, named neural basis $\mathbf{v}$ and coefficient $\mathbf{u}$.
For example, let $\mathbf{w} \in \mathbb{R}^{k^{2} \times I \times O}$ represent a convolution weight, with kernel size $k$, input channel number $I$ and output channel number $O$.
Let $p \in \{1, 2, \cdots, P\}$ denote the weight width, where the shape of $p$-width weight $\mathbf{w}_{p}$ is $k^{2} \times pI \times pO$.
Accordingly, $\mathbf{w}_{p}$ is approximated as follows:
\begin{equation}
    \mathbf{w}_{p} \approx \mathbf{v} \cdot \mathbf{u}_{p}, \qquad \mathbf{v} \in \mathbb{R}^{k^{2} \times I \times R}, \mathbf{u} \in \mathbb{R}^{R \times (p \times p O)}
\end{equation}
% \vspace{-1mm}

When $k=1$, the above format represents the approximation of fully connection layer's weight.
The weight width is controlled by adjusting the size of coefficient, while the size of neural basis is constant.
Specifically, the complete coefficient is divided into $P^{2}$ blocks, where the shape of each block is $R \times O$.
We select $p^{2}$ blocks from the complete coefficient to form the reduced coefficient and compose (\ie, multiply) it with neural basis into a $p$-width weight.

To ensure sufficient training of every parameter in the global model, we control different coefficient blocks to be trained evenly.
Thus, the selected blocks are currently the least trained ones.
Notably, we measure each block's training adequacy by the total number of local iterations it has experienced on all clients since round 1, \ie, total update times.
In general, we balance the total update times of different coefficient blocks to ensure that each block is fully trained.

For example, as illustrated in Fig. \ref{fig:neural_composition}, the coefficient $\mathbf{u} \in \mathbb{R}^{R \times (9 \times O)}$ is divided into 9 blocks (\ie, $P$=3) and the number in each block represents its current total update times.
To obtain a 2-width weight, we first extract the least trained 4 blocks (with the total update times of 6, 5, 7 and 8, respectively) from the complete coefficient and combine them into the reduced coefficient $\hat{\mathbf{u}} \in \mathbb{R}^{R \times (4 \times O)}$.
Then, $\hat{\mathbf{u}}$ is composed with the neural basis $\mathbf{v} \in \mathbb{R}^{k^2 \times I \times R}$ into an intermediate tensor whose shape is $k^2 \times I \times (4 \times O)$.
Finally, a 2-width weight $\hat{\mathbf{x}} \in \mathbb{R}^{k^2 \times (2 \times I) \times (2 \times O)}$ is obtained by reshaping this intermediate tensor.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{fig/neural composition_v2.pdf}
        \caption{The demonstration of constructing a $p$-width weight by the enhanced neural composition technique ($P$=3, $p$=2).} \label{fig:neural_composition}\vspace{-0.5cm}
\end{figure}

\begin{table}[h]
\centering
\setlength{\abovecaptionskip}{10pt}%
\setlength{\belowcaptionskip}{0pt}%
\footnotesize
\caption{Training performance within given resource constraints.}
\label{table:motivation_training_performance_completion_time}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{FL Schemes} & \multicolumn{2}{c|}{Traffic} &  \multicolumn{2}{c|}{Time} \\
\cline{2-5}
& 30GB & 60GB & 20,000s & 40,000s \\
\hline
MP \cite{diao2020heterofl} & 34.89\% & 48.92\% & 39.72\% & 50.75\% \\
\hline
Original NC \cite{mei2022resource} & 42.22\% & 51.89\% & 43.25\% & 49.37\% \\
\hline
\textbf{Enhanced NC} & \textbf{59.76\%} & \textbf{64.42\%} & \textbf{58.69\%} & \textbf{62.81\%}  \\
\hline
\end{tabular}
\end{table}

Compared to the FL schemes based on model pruning \cite{diao2020heterofl}, the neural composition technique enables every parameter in the global model to benefit from the full range of knowledge through the shared neural basis, improving the training performance.
Different from \textit{Flanc} \cite{mei2022resource} with original neural composition, enhanced neural composition allows the coefficient of all sizes to get fully trained, accelerating the training process.
To verify this improvement, we simulate a FL system with 100 clients to train the standard ResNet-18 model \cite{he2016deep} over the ImageNet dataset \cite{russakovsky2015imagenet}.
The results in Table \ref{table:motivation_training_performance_completion_time} indicate that with the given traffic consumption or completion time, the enhanced neural composition can improve the global model's test accuracy by about 16.29\% on average compared with the FL schemes based on model pruning (MP) \cite{diao2020heterofl} and original neural composition (NC) \cite{mei2022resource}.


\subsection{Adaptive Local Update}
In most synchronous FL schemes \cite{ li2021talk, mei2022resource}, the clients' local update frequencies are identical and fixed in each round.
However, due to client heterogeneity, strong clients have to wait for weak ones (\ie, stragglers) for global aggregation, incurring non-negligible waiting time and reducing the training efficiency significantly \cite{liu2023adaptive, wang2020towards}. 
To evaluate the negative impacts of stragglers, we record the completion time for one training round of each client in the simulated FL system.
As shown in Fig. \ref{fig:round_time_noadloc}, the strongest client completes one training round four times faster than the weakest client.
In other words, about 70\% of the strongest client's time is idle and wasted.

To reduce clients' idle waiting, some research \cite{li2020federated, xu2022adaptive, li2022pyramidfl} proposes adjusting the local update frequencies for different clients to balance their completion time.
On the one hand, the weaker clients perform fewer local iterations to reduce the impact of stragglers.
On the other hand, the stronger clients utilize the idle time to perform more local iterations, which helps the model converge faster.
We illustrate the completion time of each client with proper local update frequency in Fig. \ref{fig:round_time_adloc}.
It can be observed that almost every client's time is fully utilized without idle waiting.

\begin{figure}[t]
	\centering
	\subfigure[Fixed and Identical Frequency]{
		\includegraphics[width=1.6in]{fig/motivation_round_no_adloc.pdf}\label{fig:round_time_noadloc}
	}
	\subfigure[Adaptive Frequency]{
		\includegraphics[width=1.6in]{fig/motivation_round_adloc.pdf}\label{fig:round_time_adloc}
	}
 \vspace{-2mm}
	\caption{Ranked clients' completion time in one training round.}\label{fig:round_time}
	\vspace{-3mm}
\end{figure}

However, the neural composition and the local update are interconnected, and it is difficult to jointly assign proper coefficient blocks and local update frequencies for different clients.
Specifically, both the computation time and the communication time of a specific client depend on the number of coefficient blocks, which affects the determination of its local update frequency.
Meanwhile, since each client trains different blocks, various local update frequencies will also affect the balance of the blocks' total update times.

% Consequently, for a client, both the computation time of one local iteration and the communication time with the PS depend on the number of coefficient blocks, which will affect the determination of local update frequency.
% Meanwhile, the clients' local update frequencies also affect the training adequacy of different coefficient blocks.
% Accordingly, it is necessary to jointly assign proper coefficient blocks and determine the optimal local update frequency for each client to address the challenges of resource limitation and client heterogeneity.
% However, the enhanced neural composition and adaptive local update are coupled.
% Meanwhile, since each client trains different blocks, the various local update frequencies will also affect.
% Meanwhile, each client's local update frequency will also affect the training adequacy of its 
% coefficient blocks.
% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% Meanwhile, since the coefficient blocks trained by different clients are various
% With the enhanced neural composition (NC) technique, every parameter in the global model can benefit from the full range of knowledge through the shared neural basis.
% Moreover, all parameters will get fully trained by selecting the coefficient blocks appropriately, improving the training performance significantly.
% Different from the pruning-based FL schemes, where the
% Compared to model pruning (MP), where the pruned parameters cannot be optimized on clients' local data, neural composition (NC) technique enables every parameter in the global model to benefit from the full range of knowledge through the shared neural basis.

% Different from the works based on model pruning, where the pruned model parts cannot be optimized on the client's local data, the entire neural basis $\mathbf{v}$ is trained by all participating clients and the updating can be propagated to every model parameter through composition.

% With this neural composition technique, the model of any width encompasses the entire neural basis, which got trained over all clients' local dataset.
% Besides, the knowledge learned by neural basis can be propagated to all parameters in global model through neural composition, which helps the global model converge faster and better.
% Meanwhile, in the pruning-based FL schemes, the pruned model parameters cannot be optimized, leading to poor performance of global model, especially when the clients' local data is Non-IID.


% \subsection{Advantages of Neural Composition}
% % Due to the client heterogeneity, the architectures of clients' local models are heterogeneous, which will have a great impact on the global model's training performance.
% To mitigate the consumption of both computation and communication resources on edge clients, most existing works extract a smaller sub-model from the global model for local training by pruning the excessive hidden channels \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex} or the deepest layers \cite{kim2023depthfl}.
% However, the pruning is always along with the performance degradation.
% For example, if 75\% of the global model's parameters are pruned for the poor clients with low resource budgets, only 25\% of the global model's parameters can be optimized over these poor clients' local data.
% Thus, the majority (75\%) of parameters are not fully trained, leading to poor performance of the global model.




% Compared to directly pruning the model parameters, our proposed neural composition technique can improve the generalization performance of global model significantly.
% Firstly, the entire neural basis is trained by all clients and its update can be propagated to all parameters in global model, enabling every parameter to access the full range of knowledge \cite{mei2022resource}.
% Secondly, the blocks in coefficient are controlled to be evenly trained, which helps to ensure the fully optimized for all parameters in the global model.
% To verify this performance improvement, we simulate a federation with 100 clients to train the standard ResNet-18 model \cite{he2016deep} over the ImageNet dataset \cite{russakovsky2015imagenet}.
% The results shown in Table \ref{table:motivation_training_performance_completion_time} indicate that the neural composition technique can improve the global model's test accuracy by 8.73\% compared with model pruning under the same completion time.
% Despite the above advantages of the enhanced neural composition technique, the problem of synchronization barriers still hurts the training efficiency due to client heterogeneity.
% Specifically, the weak clients (\ie, stragglers) will delay the aggregation and result in long idle time for the strong clients.
% Despite the resource efficiency, 
% In order to reduce the communication cost, some existing works \cite{hsieh2017gaia} propose to perform multiple local updates on the clients before uploading the models or gradients to the PS for aggregation. However, setting the same local update frequency for each client will lead to the problem of synchronization barriers in heterogeneous systems, \ie, the stragglers (\ie, weak clients) will delay the aggregation and result in long idle time for the strong clients.
% To illustrate this, we simulate a federation with 100 clients to train the standard ResNet-18 \cite{he2016deep} over the ImageNet dataset \cite{russakovsky2015imagenet}.
% As shown in Fig. \ref{fig:round_time_noadloc}, the straggler is four times slower than the fastest client.
% In other words, 80\% of the fastest client's time is wasted.

% We observe that adjusting the number of local updates for different clients according to the heterogeneous capabilities can alleviate the above problem.
% On the one hand, the slower clients can perform fewer local iterations to reduce the impact of stragglers.
% On the other hand, the faster clients can utilize the idle time to perform more number of local updates, which helps the model converge faster.
% The testing results in Fig. \ref{fig:round_time_adloc} show that the completion time of different clients is balanced with the appropriate local update frequencies.
% However, the models trained with the different number of local iterations are discrepant, which may affect the convergence performance of global model, especially when the local models' architecture are different.
% Therefore, the existing algorithms to adjust the number of local iterations \cite{wang2018edge} cannot be directly applied in our work.

% Therefore, in order to save the limited computational resource one edge clients while ensuring the performance, we adjust the model width for each clients based on its resource budget.
% Besides, we also assign proper local update frequencies to different clients to balance their completion time as well as let the parameters of global coefficient be evenly trained.
% % However, the models trained with the different number of local iterations are discrepant, which may affect the convergence performance of global model, especially when the local models' architecture are different.
% Accordingly, we propose to jointly determine the model width and local update frequency to address the resource limitation and system heterogeneity in FL.


==> fig/content/related.tex <==
As a practical and promising approach, FL has garnered significant interest from both research and industrial communities \cite{kairouz2021advances}.
However, the training efficiency of FL often suffers from resources limitation and client heterogeneity \cite{imteaj2021survey}.
% The training efficiency of FL often suffers from resources limitation and client heterogeneity \cite{imteaj2021survey}.
In recent years, many previous works have been proposed to improve the training efficiency for FL.
To tackle the challenge of client heterogeneity, some research \cite{lai2021oort, luo2022tackling} optimizes the client sampling strategy to diminish the heterogeneity degree among participating clients.
Another approach is adjusting the local update frequencies for different clients \cite{li2020federated}, so as to balance their completion time and mitigate the effect of straggler.
% However, these approaches could not save the limited resource for FL.
However, these approaches have not been able to effectively conserve the limited resources in FL.


Compressing the transmitted gradients is a common way to alleviate the communication overhead \cite{jiang2023heterogeneity, li2021talk, wang2023federated, cui2022optimal, liu2022communication, nori2021fast}.
To further reduce the computation overhead, a natural solution is to prune the global model into a smaller sub-model for training \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, li2020lotteryfl, mugunthan2022fedltn, li2021hermes}.
Nevertheless, the compressed or pruned parameters are under-optimized in these approaches, degrading the training performance.
To address this issue, neural composition technique \cite{mei2022resource} is proposed to construct the size-adjustable models using the more efficient low-rank tensors, while enabling every parameter to learn the knowledge from all clients.
However, the global model may get insufficient training, leading to a long completion time, especially in heterogeneous edge networks.



% However, the efficiency of FL often suffers from resource limitations and client heterogeneity.
% In recent years, some works have been proposed to tackle these challenges.
% \textit{FedProx} \cite{li2020federated} and \textit{FedLamp} \cite{xu2022adaptive} propose to employ diverse local update frequencies for heterogeneous clients, so as to reduce the waiting time and enhance the training efficiency.
% However, they always ignore the resource constraints in the edge network.
% \textit{FlexCom} \cite{li2021talk} and \textit{AdaGQ} \cite{liu2022communication} adopt gradient compression technique (\eg, quantization, sparsification) to save the scarce bandwidth and adjust the compression ratios for different clients to balance their completion time.
% Nevertheless, these methods do not reduce model complexity, putting strain on limited computation resources on clients.
% Model pruning is a natural solution to save the computation and communication resources simultaneously.
% Specifically, \textit{HeteroFL} \cite{diao2020heterofl} and \textit{Fjord} \cite{horvath2021fjord} reduce the model width by pruning the excessive hidden channels.
% \textit{DepthFL} \cite{kim2023depthfl} prunes the deepest layers of the global model to reduce the model depth.
% Despite the resource efficiency, pruning restricts the clients' contributions to only a small portion of the global model, resulting in under-optimized pruned parameters and significant performance degradation.

% Different from pruning the parameters, \textit{Flanc} \cite{mei2022resource} propose to construct models at various complexities by composing two low-rank tensors, which enables every parameter in the global model to access the full range of knowledge and improves the generalization performance of the global model.
% However, the client heterogeneity still hurts the training efficiency in \textit{Flanc}.
% Furthermore, due to the separate aggregation of coefficient tensors, the global model at a specific complexity may be trained inadequately and fail to reach convergence within the given completion time.
% Therefore, none of the existing works can fully address the challenges of resource limitation and client heterogeneity while maintaining the training performance of the global model.



==> fig/content/trash.tex <==
% In this section, we define the problem of heterogeneity-aware FL with adaptive neural compostion and gredient compression. Let $t_{i}^{k, cp}$ denote the computation time for local updating of client $i$ at round $k$, which is related to the size of coefficient obviously. The larger the coefficient is, the more parameters the composed model will have, leading to longer local computation time. Considering the upload speed is usually much smaller than the download speed in FL and the parameters download time is negligible, we focus on the gredients upload time. Suppose that the gredients size of shared basis and full coefficient are $B_{v}$ and $B_{u}$, respectively, the communication time of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cm} = \frac{r_{i}^{k} (B_{v} + p_{i}^{k} B_{u}) } {b_{i}^{k}}
% \end{equation}
% where $c_{i}^{k}$ represents the upload bandwidth of client $i$ at round $k$, which is heterogeneous among clients and can change dynamically in different rounds. We define the completion time of client $i$ at round $k$ as follows:
% \begin{equation}
%     t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}
% \end{equation}
% Due to the synchronization barrier of FL, the round time (\ie, duration between two successive
% training rounds) depends on the slowest client, which can be expressed as:
% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{N}} \ t_{i}^{k}
% \end{equation}

% Our goal is to determine the optimal coefficient pruning ratios and gredients compression ratios for each client every round, so as to accelerate the training process in the heterogeneous FL setting. Accordingly, we formulate the joint optimization problem as follows:

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \epsilon \\
%     p_{i}^{k} \in \mathcal{P}, &\forall i, \forall k \\
%     0 < r_{i}^{k} \leq  1, & \forall i, \forall k 
%     \end{cases}
% \end{equation}

% The first inequality expresses the convergence requirement, where $\epsilon$ (a positive constant close to zero) is the convergence threshold of the training loss after $K$ rounds. The second set of inequalities bounds the feasible range of coefficient pruning ratios, while the third set of inequalities bounds that of gredient compression ratios.

% In this section, we define the problem of heterogeneity-aware FL with adaptive client selection and neural composition. Let $g(x_{i}^{k, h}, p_{i}^{k})$ represent the number of CPU cycles required to perform one local update, which is related to the size of coefficient. The larger the coefficient is (\ie, the more parameters the composed model have), the more CPU cycles it required to process a batch of data samples. Thus, the computation the of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cp} = \frac{\sum_{h=1}^{H} g(x_{i}^{k, h}, p_{i}^{k})} {c_{i}^{k}}
% \end{equation}

% where $c_{i}^{k}$ denote the CPU-cycle frequency for local training in round $k$. For the communication time, considering the upload speed is usually much smaller than the download speed in FL and the parameters download time can be negligible, we focus on the upload time. Suppose that the size of shared basis and full coefficient are $B_{v}$ and $B_{u}$, respectively, the communication time of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cm} = \frac{(B_{v} + p_{i}^{k}B_{u}) } {b_{i}^{k}}
% \end{equation}

% where $c_{i}^{k}$ represents the upload bandwidth of client $i$ at round $k$, which is heterogeneous among clients and can change dynamically in different rounds. Due to the synchronization barrier of FL, the round time (\ie, duration between two successive training rounds) depends on the slowest client, which can be expressed as:

% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{M}^{k}} \ t_{i}^{k}
% \end{equation}


% where $t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}$. Our goal is to select the clients involved in FL based on the statistical heterogeneity and determine the optimal size of coefficient for those selected clients, so as to accelerate the training process in the heterogeneous FL setting. Accordingly, we formulate the joint optimization problem as follows:

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \epsilon \\
%     p_{i}^{k} \in \mathcal{P}, &\forall i, \forall k \\
%     |\mathcal{M}^{k}| = M, & \forall k 
%     \end{cases}
% \end{equation}

% The first inequality expresses the convergence requirement, where $\epsilon$ (a positive constant close to zero) is the convergence threshold of the training loss after $K$ rounds. The second set of inequalities bounds the feasible range of coefficient pruning ratios. The third set of inequalities indicates that the PS selects $M$ clients participating in training at each round.

% $c_{i}^{p}$ is the computing resource consumption of one local iteration.
% $b_{v}$ and $b_{u}$

% \begin{equation}
%     t_{i}^{k, cp} = \frac{\sum_{h=1}^{\tau_{i}^{k}} g(x_{i}^{k, h}, p_{i}^{k})} {c_{i}^{k}}
% \end{equation}

% \begin{equation}
%     t_{i}^{k, cm} = \frac{(B_{v} + p_{i}^{k}B_{u}) } {b_{i}^{k}}
% \end{equation}

% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{N}} \ t_{i}^{k}
% \end{equation}

% \begin{equation}
%     t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}
% \end{equation}

% \begin{equation}
%     \mathcal{W}^{k} = \frac{1}{N} \sum_{i = 1}^{N} (t^{k} - t^{k}_{i})
% \end{equation}

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \xi  \\
%     \sum_{k = 1}^{K} \sum_{i = 1}^{N} (b_{i, v} + b_{i, u} \cdot p_{i}^{k}) \leq B  \\
%     \sum_{k = 1}^{K} \sum_{i = 1}^{N} \tau_{i}^{k} \cdot p_{i}^{k}c_{i} \leq C 
%     \end{cases}
% \end{equation}


% t_{i}^{k} = \frac{\tau_{i}^{k} g(V^{k} \cdot U^{k}_{p_{i}})} {c_{i}^{k}} + \frac{h(V) + h(U^{k}_{p_{i}}) } {b_{i}^{k}}, & \forall i, k \\

% \subsection{Federated Learning Basics}
% Consider a loose federation of $N$ clients $\mathcal{N} = \{1, 2, \cdots, N \}$ coordinated by the PS.
% Each client $n \in \mathcal{N}$ holds its local dataset $D_{n} = \{\zeta_{i}^{n}\}_{i=1}^{|D_{n}|}$, where $\zeta_{i}$ denotes a data sample from $D_{n}$.
% Further, we represent the loss function as $\mathcal{L}(\mathbf{x}; \zeta)$, which measures how well the model $\mathbf{x}$ perform on data sample $\zeta$.
% Therefore, the local loss function of client $n$ is defined as:

% \begin{equation}
%     F_{n}(\mathbf{x}) \triangleq \mathbb{E}_{\zeta \thicksim D_{n}} [\mathcal{L}(\mathbf{x}; \zeta)] 
% \end{equation}

% The global loss function is a linear combination of all $N$ clients, and the goal of FL is to train a high-quality model $\mathbf{x}^{*}$ to minimize the value of global loss function, which can be defined as follows:

% \begin{equation} \label{eq:fl_goal}
%     \mathbf{x}^{*} \triangleq  \mathop{\arg\min}_{\mathbf{x}} F(\mathbf{x}) = \mathop{\arg\min}_{\mathbf{x}} \frac{1}{N} \sum_{n=1}^{N} F_{n} (\mathbf{x})
% \end{equation}

% FedAvg \cite{mcmahan2017communication} is the pioneer and also the most widely used FL method to solve the problem in Eq. \eqref{eq:fl_goal}.
% In each round $h \in \{1, 2, \cdots, H\}$, the PS randomly selects $K$ clients to participate in training and sends the global model $\mathbf{x}^{h}$ to the selected clients $\mathcal{N}^{h} \subseteq  \mathcal{N}$.
% Then, each client $n \in \mathcal{N}^{h}$ performs local update for $\tau$ iterations.
% Let $\mathbf{x}^{h}_{n} (t)$ denote the local model of client $n$ at iteration $t$ in round $h$.
% For the mini-batch stochastic gradient descent (SGD) algorithm, a local update step can be expressed as follows:

% \begin{equation}
%     \mathbf{x}^{h}_{n} (t+1) = \mathbf{x}^{h}_{n} (t) - \eta \nabla F_{n} (\mathbf{x}^{h}_{n} (t); \xi_{n}^{h, t})
% \end{equation}
% where $\xi_{n}^{h, t}$ denotes a random data batch from the local dataset $D_{n}$ and $\eta$ is the learning rate.
% Finally, the PS collects the updated model $\mathbf{x}^{h}_{n}$ from the participating clients and aggregate them to the latest global model for further training, \ie, $ \mathbf{x}^{h+1} = \frac{1}{N} \sum_{n=1}^{N} \mathbf{x}^{h}_{n} (\tau) $.




% \subsection{Impact of model width}

% As the most common terminal device, mobile phones are the primary data source and usually participate in training as clients.
% However, in practice, these phones are generally resource-constrained with poor computing power, so that they may not be able to afford the overhead to train the complete model.
% Therefore, it is necessary to reduce the model complexity for these poor clients, which can be achieved by reducing the model's depth (\ie, number of layers) or width (\ie, number of hidden channels) \cite{diao2020heterofl, horvath2021fjord, kim2023depthfl}.
% In this work, we adjust the model complexity by modulating the model width, which can reduce parameters and memory footprint during training more effectively compared to reduing model depth \cite{mei2022resource}.

% We can significantly reducing the computing complexities and training overhead of a DNN model, but it usually comes with performance degradation.
% To verify this phenomenon, we construct a CNN model with three 3$\times$3 convolutional layers and one fully-connected layer.
% We reduce the number of hidden channels in each layer by 0.25, 0.5, 0.75 and 1.0 times, respectively, and train these models in different width over CIFAR-10 to record their training overhead and test accuracy.
% The results shown in Table. xx indicate that the smaller the model width, the less training overhead, but the lower the accuracy.
% For instance, xxxx.
% To minimize the performance degradation, the model width should be as large as possible within the clients' computing power.

% \begin{table}[h]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_with}
% 	\begin{tabular}{c|ccc}
% 		\hline
% 		Width & \tabincell{c}{Memory \\ Footprint (MB)} & FLOPs (M) & \tabincell{c}{Test \\ Accuracy (\%)} \\
% 		\hline
% 		0.25$\times$ & -- & -- & -- \\
% 		0.5$\times$  & -- & -- & -- \\
% 		0.75$\times$ & -- & -- & -- \\
% 		1.0$\times$  & -- & -- & -- \\
% 		\hline
% 	\end{tabular}
% \end{table}
% % To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} propose to prune the global model into a small one.
% % Nevertheless, the pruned parameters cannot be optimized on client's local data, resulting in poor performance.

% % In order to reduce the model complexity without much performance degradation, we decompose the model into two low-rank tensors, named neural basis and coefficient, and only prune the coefficient.
% % The entire neural basis is trained by all clients and the update can be propagated to every model parameter after recomposition, ensuring high model performance.
% % To varify the effectiveness of the proposed approach, we train the models in different complexities (\ie, GPU memory occupancy) over ImageNet-100.
% % The results shown in Fig. \ref{fig:motivation_acc_memory} indicate that the smaller the model, the worse the performance (\ie, accuracy).
% % Besides, it can be observed that the composited model achieves about 5.1\% higher accuracy than the pruned model at the same computing complexity. 

% % There is still one issue when .
% % According to related research, most people use cheap mobile phones with low computing power.
% % Therefore, most clients can only train a small part of coefficient, resulting that the total updating time varies greatly between different coefficient parts.
% % This training inconsistency in updating times may have a negative impact on the convergence performance.
% % We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% % The results in Fig. \ref{fig:motivation_acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% % To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:motivation_acc_hetero}.





% % In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}. 
% % However, the computing capabilities of each clinet may vary significantly and even dynamically in practice \cite{diao2020heterofl}.

% % In practice, the computing capabilities of clients may significantly heterogeneous and even vary dynamically \cite{diao2020heterofl}.

% % In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}, which means a same computational complexity for all clients.
% % Nevertheless, the computing capabilities of clients are generally heterogeneous and may even change dynamically in practice, leading to a long system waiting time in synchronous manner \cite{xu2022adaptive}.
% % Moreover, as the model size continues to increase (\eg, the parameters number of GPT-3 reaches 175 billion \cite{floridi2020gpt}), resource-constrained edge clients may not be able to afford the training overhead (\eg, memory, energy).
% % To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} prune or quantify the global model into a submodel for each client based on its computing capability, so as to alleviate the synchronization barrier issue and diminish the resource consumption.
% % However, for the prune-based methods, the unpruned parameters cannot be optimized in clients' local data, leading to poor performance of global model.
% % Besides, the quantify-based methods will introduce model errors, which also diminishes the performance.
% % Instead of pruning the global model into local ones, FLANC \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% % construct models at various complexities by composing different neural components (\ie, tensors).
% % Instead of pruning or 

% % Different from the above methods, Flanc \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% % The neural basis is trained by all participating clients and the updating can be propagated to every model parameter through neural composition.
% % We trained models in different complexities (\ie, GPU memroy usage) over ImageNet-100 by HeteroFL and Flanc, respectively. 
% % The results shown in Fig. \ref{fig:acc_memory} indicate that the composited model can achieve higher accuracy compared to the pruned model with the same complexity.

% % \begin{figure}[h]
% % 	\centering
% % 	\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}
% % 	\caption{Model performance of different methods.}\label{fig:acc_memory}
% % 	\vspace{-3mm}
% % \end{figure}

% % \begin{figure}[h]
% % 	\centering
% % 	\subfigure[Different computing complexities]{
% % 		\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}\label{fig:motivation_acc_memory}
% % 	}
% % 	\subfigure[Different hetergeneity levels]{
% % 		\includegraphics[width=1.6in]{fig/motivation_acc_hetero.pdf}\label{fig:motivation_acc_hetero}
% % 	}
% % 	\caption{The model accuracy in different conditions.}\label{fig:motivation_model_accuracy}
% % 	\vspace{-3mm}
% % \end{figure}






% \subsection{Impact of local update frequency}
% % Even if FLANC \cite{mei2022resource} enables clients to train complexity-adjustable model.
% % In general, the above techniques are able to custom the model's computing complexity according to clients' computing power.
% % There is still one issue to perform FL in edge computing system.
% % By pruning the coefficient, we can custom the model's computing complexity according to clients' computing power.
% % However, there is still one issue to 
% % However, the edge clients are not only heterogeneous in terms of computing capability, but also in terms of communication capability (\eg, bandwidth) \cite{wang2022accelerating}.
% % As shown in Fig. \ref{fig:round_time_noadloc}, although the local updating time is approximately equal among all clients, the clients with slow communication speed can easily become the bottleneck and lead to long idle time for fast clients. 

% There is still one issue to perform FL in edge computing system.
% Since the clients' capabilities (\eg, computing power, bandwidth) are highly heterogeneous and even time-varying, the stragglers will delay the aggregation and result in long idle time for fast clients.
% As shown in Fig. \ref{fig:round_time_noadloc}, the time cost of the fastest client in one round is only 20\% of the slowest client.
% In other word, 80\% of the fastest client' time is wasted.

% In order to alleviate this problem, we can adjust the numbers of local iterations for different clients, and the effect is illustrated in Fig. \ref{fig:round_time_adloc}.
% On the one hand, the slower can perform fewer local iterations to reduce the impact of stragglers.
% On the other hand, the faster clients can utilize the idle time to perform more local iterations, which helps the model converge faster.
% However, the models trained with different number of local iterations are discrepant, which may affect the convergence performance of global model, especially when the local models' architecture are different.
% Therefore, the existing algorithms to adjust the number of local iterations \cite{wang2018edge} cannot be directly applied in our work. 

% \begin{figure}[h]
% 	\centering
% 	\subfigure[Fixed Updating Frequency]{
% 		\includegraphics[width=1.6in]{fig/motivation_roundtime_noadloc.pdf}\label{fig:round_time_noadloc}
% 	}
% 	\subfigure[Adaptive Updating Frequency]{
% 		\includegraphics[width=1.6in]{fig/motivation_round_adloc.pdf}\label{fig:round_time_adloc}
% 	}
% 	\caption{Ranked clients' time cost in one round.}\label{fig:round_time}
% 	\vspace{-3mm}
% \end{figure}

% % There is still one issue when trianing complexity-adjustable in mobile phones.
% % According to related research, most people use cheap mobile phones with low computing power.
% % Therefore, most client can only train a small part of coefficient, which results that the updating time varies greatly between different clients.
% % This training inconsistency may have a negative impact on the convergence performance.
% % We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% % The results in Fig. \ref{fig:acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% % To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:acc_hetero}.

% However, running these models on edge clients (\eg, smartphones) may encounter performance degradation issues due to the limited computational and communication resources. 

% As the most common terminal device, mobile phones are the primary data source and usually participate in training as clients.
% However, in practice, these phones are generally resource-constrained with poor computing power, so that they may not be able to afford the overhead to train the complete model.

% \begin{table}[t]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_with}
% 	\begin{tabular}{c|ccccc}
% 		\hline
% 		Width & Parameters(M) & Size(MB) & \tabincell{c}{Memory \\ Footprint(MB)} & FLOPs(M) & \tabincell{c}{Test \\ Accuracy(\%)} \\
% 		\hline
% 		0.25$\times$ & -- & -- & -- & -- & -- \\
% 		0.5$\times$  & -- & -- & -- & -- & -- \\
% 		0.75$\times$ & -- & -- & -- & -- & -- \\
% 		1.0$\times$  & -- & -- & -- & -- & -- \\
% 		\hline
% 	\end{tabular}
% \end{table}

% To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} propose to prune the global model into a small one.
% Nevertheless, the pruned parameters cannot be optimized on client's local data, resulting in poor performance.

% In order to reduce the model complexity without much performance degradation, we decompose the model into two low-rank tensors, named neural basis and coefficient, and only prune the coefficient.
% The entire neural basis is trained by all clients and the update can be propagated to every model parameter after recomposition, ensuring high model performance.
% To varify the effectiveness of the proposed approach, we train the models in different complexities (\ie, GPU memory occupancy) over ImageNet-100.
% The results shown in Fig. \ref{fig:motivation_acc_memory} indicate that the smaller the model, the worse the performance (\ie, accuracy).
% Besides, it can be observed that the composited model achieves about 5.1\% higher accuracy than the pruned model at the same computing complexity. 

% There is still one issue when .
% According to related research, most people use cheap mobile phones with low computing power.
% Therefore, most clients can only train a small part of coefficient, resulting that the total updating time varies greatly between different coefficient parts.
% This training inconsistency in updating times may have a negative impact on the convergence performance.
% We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% The results in Fig. \ref{fig:motivation_acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:motivation_acc_hetero}.


% In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}. 
% However, the computing capabilities of each clinet may vary significantly and even dynamically in practice \cite{diao2020heterofl}.

% In practice, the computing capabilities of clients may significantly heterogeneous and even vary dynamically \cite{diao2020heterofl}.

% In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}, which means a same computational complexity for all clients.
% Nevertheless, the computing capabilities of clients are generally heterogeneous and may even change dynamically in practice, leading to a long system waiting time in synchronous manner \cite{xu2022adaptive}.
% Moreover, as the model size continues to increase (\eg, the parameters number of GPT-3 reaches 175 billion \cite{floridi2020gpt}), resource-constrained edge clients may not be able to afford the training overhead (\eg, memory, energy).
% To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} prune or quantify the global model into a submodel for each client based on its computing capability, so as to alleviate the synchronization barrier issue and diminish the resource consumption.
% However, for the prune-based methods, the unpruned parameters cannot be optimized in clients' local data, leading to poor performance of global model.
% Besides, the quantify-based methods will introduce model errors, which also diminishes the performance.
% Instead of pruning the global model into local ones, FLANC \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% construct models at various complexities by composing different neural components (\ie, tensors).
% Instead of pruning or 

% Different from the above methods, Flanc \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% The neural basis is trained by all participating clients and the updating can be propagated to every model parameter through neural composition.
% We trained models in different complexities (\ie, GPU memroy usage) over ImageNet-100 by HeteroFL and Flanc, respectively. 
% The results shown in Fig. \ref{fig:acc_memory} indicate that the composited model can achieve higher accuracy compared to the pruned model with the same complexity.

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}
% 	\caption{Model performance of different methods.}\label{fig:acc_memory}
% 	\vspace{-3mm}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\subfigure[Different computing complexities]{
% 		\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}\label{fig:motivation_acc_memory}
% 	}
% 	\subfigure[Different hetergeneity levels]{
% 		\includegraphics[width=1.6in]{fig/motivation_acc_hetero.pdf}\label{fig:motivation_acc_hetero}
% 	}
% 	\caption{The model accuracy in different conditions.}\label{fig:motivation_model_accuracy}
% 	\vspace{-3mm}
% \end{figure}

% Even if FLANC \cite{mei2022resource} enables clients to train complexity-adjustable model.
% In general, the above techniques are able to custom the model's computing complexity according to clients' computing power.
% There is still one issue to perform FL in edge computing system.
% By pruning the coefficient, we can custom the model's computing complexity according to clients' computing power.
% However, there is still one issue to 
% However, the edge clients are not only heterogeneous in terms of computing capability, but also in terms of communication capability (\eg, bandwidth) \cite{wang2022accelerating}.
% As shown in Fig. \ref{fig:round_time_noadloc}, although the local updating time is approximately equal among all clients, the clients with slow communication speed can easily become the bottleneck and lead to long idle time for fast clients. 
% There is still one issue to perform FL in edge computing system.
% Since the clients' capabilities (\eg, computing power, bandwidth) are highly heterogeneous and even time-varying, 

% As shown in Fig. \ref{fig:round_time_noadloc}, the time cost of the fastest client in one round is only 20\% of the slowest client.

% There is still one issue when trianing complexity-adjustable in mobile phones.
% According to related research, most people use cheap mobile phones with low computing power.
% Therefore, most client can only train a small part of coefficient, which results that the updating time varies greatly between different clients.
% This training inconsistency may have a negative impact on the convergence performance.
% We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% The results in Fig. \ref{fig:acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:acc_hetero}.

% Moreover, the heterogeneity among the clients, \ie, the computing power and communication capacity of different edge clients is significantly varied, will also have a great impact on training efficiency.
% For example, the hardware manufacturer typically configure 
% For example, mobile manufacturers typically configure multiple processors (\eg, Snapdragon, Apple A-series chips) on the client to cater to the diverse needs of customers, however, resulting in inconsistent completion time for model training.
% Besides, the computing power and communication capacity of different edge clients is significantly varied, which will have a great impact on training efficiency.
% For example, there can be a tenfold difference in CPU frequency or bandwidth for the edge devices \cite{xu2022adaptive}.
% In synchronous mode, clients with faster training and/or communication speed often have to wait the stragglers for global aggregation, resulting in a longer or even unacceptable completion time of model training.
% In addition, due to the intrinsic and/or external conditions, such as ambient temperatures, CPU states,
% network connections to the server and so on, the per-round computing time and communication time at each client may vary significantly.
% The different network connection methods (\eg, 4G, 5G and WIFI) of the client also affect the communication cost of model transmission during the training process\cite{}.
% Besides, the availability and connectivity of edge clients may change over time, \ie, network dynamics.
% For instance, the smartphone can freely join or exit the training process. 
% The addition of clients will increase the scale and data diversity of training, while the withdrawal of clients may lead to data loss during training, leading to the performance degradation of the model training.

% Moreover, the heterogeneity among the clients, \ie, the computing power and communication capacity of different edge clients is significantly varied, will also have a great impact on training efficiency.
% For example, the hardware manufacturer typically configure 
% For example, mobile manufacturers typically configure multiple processors (\eg, Snapdragon, Apple A-series chips) on the client to cater to the diverse needs of customers, however, resulting in inconsistent completion time for model training.

% The different network connection methods (\eg, 4G, 5G and WIFI) of the client also affect the communication cost of model transmission during the training process\cite{}.
% Besides, the availability and connectivity of edge clients may change over time, \ie, network dynamics.
% For instance, the smartphone can freely join or exit the training process. 
% The addition of clients will increase the scale and data diversity of training, while the withdrawal of clients may lead to data loss during training, leading to the performance degradation of the model training.

% For example, performing one mini-batch SGD on standard ResNet-18\footnote{Image resolution is 3$\times$144$\times$144, batch size is 32.} with NVIDIA Jetson TX2\footnote{A commercial edge embedded AI computing device. More details are available at https://www.nvidia.cn/autonomous-machines/embedded-systems} takes xxx minutes and consumes xx\% of the battery.


% Different from pruning the global model directly, \textit{Flanc} \cite{mei2022resource} proposes to construct the models in different width by multiplying the neural basis with different coefficient.
% The neural basis is shared by all clients, which enables every parameter in global model to access the full range of knowledge of all clients, improving the performance of global model.
% Despite the improvement, \textit{Flanc} only aggregates the coefficients with the same shape, thus the learned coefficient will be biased towards the data distribution of corresponding particular clients set, which hurts the generalization performance of the global model when the local datasets are Non-IID.
% To verify this phenomenon, we test the \textit{HeteroFL} and \textit{Flanc} by training CNN on CIFAR-10 under three different Non-IID levels, denoted by \textit{low}, \textit{medium} and \textit{high}, respectively. 
% The results shown in Table \ref{table:motivation_training_heterogeneous_models} indicate that \textit{Flanc} achieves better performance than \textit{HeteroFL}, but the test accuracies of both \textit{Flanc} and \textit{HeteroFL} are significantly decreased as the Non-IID level increases.
% To this end, we design a novel neural composition technique to aggregate the coefficients in different shape into a global one and let the parameter in global coefficient be evenly trained, so as to improve the training robustness against Non-IID data.
% By Table \ref{table:motivation_training_heterogeneous_models}, the global model can achieve the best test accuracy with our proposed technique. 


% Therefore, it is necessary to reduce the model complexity for these resource-constrained clients by reducing the model's depth (\ie, number of layers) \cite{kim2023depthfl} or width (\ie, number of hidden channels) \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex}.
% In this work, we mainly focus on adjusting the model complexity by modulating the model width, which can reduce parameters and memory footprint during raining more effectively compared to reducing model depth \cite{mei2022resource}.

% Some techniques (\eg, model pruning) can significantly reduce the computing complexities and training overhead of a DNN model, but it usually comes with performance degradation.
% Reducing the model width can significantly reduce the computing complexities and training overhead, but it usually comes with performance degradation.
% To evaluate the impact of model width on FL training, we construct a CNN model with three 3$\times$3 convolutional layers and one fully-connected layer, where each convolutional layer has 64, 128 and 128 hidden channels, respectively.
% We reduce the model width by 0.25, 0.5, 0.75 and 1.0 times, and record the model's training overhead and test accuracy over CIFAR-10, respectively.
% The results in Table. \ref{table:motivation_models_in_different_width} indicate that the smaller the model width, the less training overhead, but the lower the accuracy.
% For instance, the 1.0-width model needs about 15 times more FLOPs to process an image than the 0.25-width model, but its test accuracy is 6.29\% higher.
% To minimize the performance degradation, the model width should be as large as possible within the clients' computing power.

% \begin{table}[t]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_width}
% 	\begin{tabular}{c|cccc}
% 		\hline
% 		Width & 0.25$\times$ & 0.5$\times$ & 0.75$\times$ & 1.0$\times$ \\
% 		\hline
% 		Parameters(K) & 34.87 & 97.29 & 187.4 & 305.16 \\
% 		Size(MB) & 0.13 & 0.37 & 0.72 & 1.16 \\
% 		Memory Footprint(MB) & 22.35 & 59.64 & 68.69 & 92.16 \\
% 		FLOPs(M) & 7.68 & 29.52 & 65.51 & 115.65 \\
% 		Test Accuracy(\%) &  81.09 & 85.05 & 86.65 & 87.38 \\
% 		\hline
% 	\end{tabular}
% \end{table}

% In FL, each client performs model training on its local dataset and then sends the updated model to the parameter server (PS). 
% Once receiving the local updated models from clients, PS will aggregate them and distribute the fresh global model to the clients for the next round of training. 
% The whole process continues until the global model converges.
% As the field continues to evolve, FL holds significant potential for advancing the capabilities of edge computing and enabling intelligent applications in diverse domains, such as healthcare, autonomous vehicles, and smart cities \cite{rahman2021challenges}.

% Despite the advantages of FL, the growing complexity (\eg, the parameter size or architecture) of deep neural networks (DNNs) incurs a large amount of computation and communication overhead during model training.
% Computation and Communication Resource Limitation.
% Mobile Phones cannot train the DNNs models
% iPhone....

% In order to reduce the communication cost, some existing works \cite{hsieh2017gaia} propose to perform multiple local updates on the clients before uploading the models or gradients to the PS for aggregation. However, setting the same local update frequency for each client will lead to the problem of synchronization barriers in heterogeneous systems, \ie, the stragglers (\ie, weak clients) will delay the aggregation and result in long idle time for the strong clients.


% Related Works:
% 1) Local Update Frequency Optimization
% 2) Gradient Compression
% 3) Model Pruning

% Introduce Neural Composition

% Nevertheless, the system heterogeneity is still a challenge

% We propose a novel framework to ....
% Firstly, the computation resource is always constrained on edge clients, such as smartphones and Internet of Things (IoT) devices.
% For example, the floating-point operations per second (FLOPS) of an iPhone14 is 18.2$\times$ smaller than that of desktop GPU RTX3090.

% Different from data centers where the server clusters communicate with each other over high-speed LANs, edge clients usually communicate with PS through WANs, whose bandwidth is much lower than that of LANs.

% Consequently, the frequent model transmissions will result in a long communication time, potentially becoming a bottleneck in the training process.
% On the other hand, 
% For instance, a standard ResNet-18 \cite{he2016deep} consists of 11.68 million parameters and requires 27.29 billion floating-point operations (FLOPs) to classify a single image, making the local update process extremely slow or even infeasible on edge clients \cite{jiang2022fedmp}.


% For example, smartphones are an important data source, yet their computation resource is severely limited (\eg, CPU power, RAM, battery).
% To perform efficient model training over the weak clients like smartphones, \textit{HeteroFL} \cite{diao2020heterofl} prunes 93.75\% of the parameters from the complete model.
% In other words, only 6.25\% of the parameters are optimized while the majority of the parameters can not benefit from the smartphones' local data, leading to poor training performance of the complete model.

% Nevertheless, pruning restricts the clients' contributions to only a small portion of the global model, resulting in under-optimized pruned parameters and significant performance degradation.
% For example, 

% However, \textit{Flanc} only aggregates coefficients with the same shape, which will introduce the training bias towards specific client sets. 
% This limitation negatively impacts the generalization performance of the global model, particularly when dealing with non-independent and non-identically distributed (Non-IID) local datasets.

%and making the training process inefficient.
% However, the upload speed of this client is very slow, which will lead to long completion time, delay the aggregation step and make the training process inefficient.
% In synchronous mode, clients with fast computation and/or communication speed often have to wait for the stragglers for global aggregation, resulting in a longer or even unacceptable completion time.
% For example, due to the expensive price, the high-performance clients are typically rare in the edge system.
% The largest coefficient can only benefit from a few powerful clients, thus the largest global model may not convergence within the given completion time, leading to poor training performance.

% 1) \textit{Limited Computation Resource.}
% The 
% For example, the standard ResNet-18 \cite{he2016deep} contains 11.68 million parameters and requires 27.29 billion floating-point operations (FLOPs) to classify a single image, making the local update process extremely slow or even infeasible on edge clients \cite{jiang2022fedmp}.
% 2) \textit{Limited Communication Resource.}
% Besides, the bandwidth of wide area networks (WANs) between the parameter server (PS) and edge clients is much (\eg, 15$\times$) lower than that of local area networks (LANs) within the data centers \cite{wang2021resource}. 
% Consequently, the frequent model transmissions will result in a long communication time, potentially becoming a bottleneck in the training process.
% 3) \textit{Client Heterogeneity.}
% Moreover, the computing power and communication capacity of different edge clients is significantly varied.
% For example, there can be a tenfold difference in CPU frequency or bandwidth for the edge clients \cite{xu2022adaptive}.
% In synchronous mode, clients with fat computation and/or communication speed often have to wait for the stragglers for global aggregation, resulting in a longer or even unacceptable completion time.

% Despite the advantages of FL, the growing complexity (\eg, the parameter size or architecture) of deep neural networks (DNNs) incurs a large amount of computation and communication overhead during model training.
% For example, the standard ResNet-18 \cite{he2016deep} contains 11.68 million parameters and requires 27.29 billion floating-point operations (FLOPs) to classify a single image, making the local update process extremely slow or even impossible on the resource-constrained edge clients \cite{jiang2022fedmp}.
% Besides, the bandwidth of wide area networks (WANs) between the parameter server (PS) and edge clients is much (\eg, 15$\times$) lower than that of local area networks (LANs) within the data centers \cite{wang2021resource}. 
% Consequently, the frequent model transmissions will result in a long communication time, potentially becoming a bottleneck in the training process.




% In order to simultaneously save the computation and communication resources in FL, a natural solution is to prune the global model into the smaller sub-models according to the clients' resource constraints \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl}.
% For example, \textit{HeteroFL} \cite{diao2020heterofl} prunes excessive hidden channels in each layer, while \textit{DepthFL} \cite{kim2023depthfl} prunes the deepest layers from the global model.
% Nevertheless, pruning restricts the clients' contributions to only a small portion of the global model, resulting in under-optimized pruned parameters and significant performance degradation.

% To address this issue, \textit{Flanc} \cite{mei2022resource} proposes to approximate the deep learning model as the product of two low-rank tensors, named neural basis and coefficient.
% The model at different widths can be constructed by composing (\ie, multiplying) the neural basis with coefficients of different shapes.
% The entire neural basis is trained by all clients and its update can be propagated to every parameter of the global model through composition, allowing the full global model to benefit from the knowledge of all clients.
% However, \textit{Flanc} only aggregates coefficients with the same shape, which will introduce the training bias towards specific client sets. 
% This limitation negatively impacts the generalization performance of the global model, particularly when dealing with non-independent and non-identically distributed (Non-IID) local datasets.
% However, \textit{Flanc} only aggregates the coefficients with the same shape and the learned coefficient will be biased towards the corresponding particular clients set, which hurts the generalization performance of the global model especially when the local datasets are not independent and identically distributed (Non-IID).
% To eliminate the training deviation of coefficients, we propose to adopt a novel neural composition technique that aggregates the coefficients with different shapes into a global one, enabling every parameter in the global model to be fully trained.


% In this way, the entire neural basis is trained by all clients and its obtained update can be propagated to every parameter of the global model through composition. 
% However, \textit{Flanc} only aggregates the coefficients with the same shape, which makes the learned coefficient biased towards the corresponding particular group of clients. 
% However, the computing power and communication capacity of different edge clients is significantly varied, which will have a great impact on training efficiency.
% Despite reducing model complexity to save computing and communication resources through neural composition,
% Despite the resource saving by neural composition technique,
% In addition to the resource limitation, FL also faces two critical challenges, \ie, client heterogeneity and dynamics, which will have a great impact on training efficiency.
% Firstly, the computing power and communication capacity of different edge clients is significantly varied.
% For example, there can be a tenfold difference in CPU frequency or bandwidth for the edge clients \cite{xu2022adaptive}.
% Besides, due to the dynamic of network condition and the instability of clients states, the per-round computing time and communication time at each client may also vary significantly.
% In synchronous mode, clients with fast training and/or communication speed often have to wait for the stragglers for global aggregation, resulting in a longer or even unacceptable completion time of model training.



% In order to synchronize the training process of heterogeneous clients in a dynamic environment, some works propose to control each participating client's computing time \cite{li2020federated, xu2022adaptive, li2022pyramidfl} or communication time \cite{li2021talk, cui2022optimal, jiang2022adaptive}.
% For example, \textit{FedProx} \cite{li2020federated} adaptively determines proper local update frequency for each participating client based on its constrained resource, so as to balance the computing time of different clients.
% \textit{FlexCom} \cite{li2021talk} adopts the model compression technique (\eg, quantization or sparsification) to alleviate the communication load and dynamically adjusts the compression ratio for each participating client on the basis of time-varying link speed, thus balancing the communication time across different clients.
% However, all of these schemes require the participating clients to train the complete model, which will strain the limited computation resources available on edge clients.

% \begin{table}[t]
% \centering
% \setlength{\abovecaptionskip}{10pt}%
% \setlength{\belowcaptionskip}{0pt}%
% \footnotesize
% \caption{Comparison of different FL schemes.}
% \label{table:FL_schemes_comparison}
% \begin{tabular}{c|c|c|c}
% \hline
% FL schemes & \tabincell{c}{Resource \\ Efficiency} & \tabincell{c}{Heterogeneity \\ and Dynamic} & \tabincell{c}{Performance \\ 
% Guarantee}\\
% \hline
% \tabincell{c}{Model \\ Pruning } \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex} & \checkmark & \ding{55} & \ding{55} \\
% \hline    
% \tabincell{c}{Gradient \\ Compression} \cite{li2021talk, cui2022optimal, jiang2022adaptive} & \ding{55} & \checkmark & \ding{55}  \\
% \hline
% \tabincell{c}{Frequency \\ Optimization} \cite{li2020federated, xu2022adaptive, li2022pyramidfl}  & \ding{55} & \checkmark & \checkmark\\
% \hline
% \tabincell{c}{\textbf{Proposed} \\ \textbf{Framework}}  & \checkmark & \checkmark & \checkmark \\
% \hline
% \end{tabular}
% \end{table}


% As summarized in Table \ref{table:FL_schemes_comparison}, the existing works cannot fully address the challenges of resource limitation, client heterogeneity and dynamics with the performance guarantee.
% To this end, we propose a novel FL framework, named Heroes, which investigates the benefits of neural composition technique and adaptive local update frequency so as to reduce the resource cost and eliminate the idle time incurred by synchronization.
% However, the neural composition and local update frequency are coupled. 
% Concretely, the completion time depends on the size of composed model, which affects the determination of local update frequency.
% Meanwhile, the local update frequency also affects the training adequacy of each parameter.
% Therefore, \textit{it is necessary yet challenging to jointly assign proper coefficient blocks and determine the optimal local update frequency for each client.}
% Our contributions are summarized as follows:
% Concretely, we modify the model width by controlling the size of coefficient tensor for each client based on its computing power to save both the limited computing and communication resources.
% Additionally, we adjust the local update frequencies for heterogeneous clients to balance their completion time and let the parameters in coefficient tensor be evenly trained.
% \textit{Nevertheless, how to assign appropriate coefficient and local update frequencies to heterogeneous clients remains an important challenge in Heroes.}
% \begin{itemize}
%     \item We propose a novel FL framework, called Heroes, which overcomes the challenges of resource limitation as well as client heterogeneity and dynamic by adaptive neural composition and local update.
%     \item We theoretically analyzed the convergence of Heroes and formulated the optimization problem. Guided by the convergence bound, we propose a control algorithm to adjust the coefficient tensor and determine the local update frequency for each participating client.
%     \item The experimental results demonstrate that Heroes can speedup the training process by up to 2.4$\times$ and improve the test accuracy by about 8.75\% compared with the baselines.
    % \item We conduct extensive experiments on typical models and real-world datasets to show the effectiveness and efficiency of our proposed framework. The experimental results demonstrate that Heroes can speedup the training process by up to 2.4$\times$ and improve the test accuracy by about 8.75\% compared with the baselines.
% \end{itemize}

% The rest of this paper is organized as follows. 
% Section \ref{sec:motivation} introduces the background and motivation for our work.
% Section \ref{sec:prelim} states the process of the proposed framework.
% Section \ref{sec:analysis} provides the convergence analysis of xxx.
% Section \ref{sec:algorithm} formulates the optimization problem and designs the control algorithm.
% Section \ref{sec:evaluation} presents the evaluation results.
% Section \ref{sec:related} reviews related work and we conclude this paper in Section \ref{sec:conclusion}.
% \textit{FedAvg} \cite{mcmahan2017communication} is the pioneer and also the most widely used FL method to solve the problem in Eq. \eqref{eq:fl_goal}.

% Let $\mathbf{x}^{h}$ denote the global model in round $h$. 
% Generally, complex models (\eg, deeper architecture or more number of parameters) tend to provide better training performance because they have stronger expressive power \cite{zhang2021understanding}. 
% However, training these models will consume excessive computational and communication resources, leading to long completion time or even inability to run on edge clients.

% According to the low-rank decomposition techniques, $\mathbf{w}$ can be approximated as $\mathbf{w} \approx \mathbf{v} \cdot \mathbf{u}$, where $\mathbf{v} \in \mathbb{R}^{k^{2} \times PI \times R}$ and $\mathbf{u} \in \mathbb{R}^{R \times PO}$.
% It means that we can obtain the models in different widths by adjusting the shape of $\mathbf{v}$ or $\mathbf{u}$.
% Thus, the model' width is related to the shape of $\mathbf{v}$ or $\mathbf{u}$.
% Suppose that we reduce the model width by up to $P$ times, 
% Based on the low-rank decomposition technique \cite{phan2020stable}, ]
% The weights in different widths only differ on the shape of coefficient while the shape of basis is constant.
% The weight's width depends on the shape of coefficient, and the shape of basis is constant.
% Thus, we reduce the model width by only reducing the size of coefficient $\mathbf{u}$.
% Thus, we can control the weight's width by adjusting the coefficient.
% Thus, the weight's width can be controlled by adjusting the size of coefficient.

% We select $p^{2}$ parts of coefficient to composite with neural basis to obtain the $p$-width model.

% We measure the amount of training each block has obtained by the total local iterations it has experienced on all clients since round 1, \ie, total update times.
% For the convenience of expression, we utilize $c_{i}^{h}$ to represent the total update times of block $i$ in round $h$.
% Notably, to ensure the sufficient training for all coefficient blocks, the selected $p^{2}$ blocks are the ones with the least training.
% Instead of pruning model parameters directly, 
% Compared to the prune-based schemes, where the pruned model parts cannot be optimized, this approach can improve the training stability and performance, beacuse the entire neural basis $\mathbf{v}$ get update over all clients' local data (\ie, learn knowledge from all clients) and the update can be propagated to every model parameter through composition.
